Consent in Crisis: The Rapid Decline of the AI Data Commons

General-purpose artificial intelligence (AI) systems are built on massive swathes of public web data, assembled into corpora such as C4, RefinedWeb, and Dolma. To our knowledge, we conduct the first, large-scale, longitudinal audit of the consent protocols for the web domains underlying AI training corpora. Our audit of 14,000 web domains provides an expansive view of crawlable web data and how codified data use preferences are changing over time. We observe a proliferation of AI-specific clauses to limit use, acute differences in restrictions on AI developers, as well as general inconsistencies between websites' expressed intentions in their Terms of Service and their robots.txt. We diagnose these as symptoms of ineffective web protocols, not designed to cope with the widespread re-purposing of the internet for AI. Our longitudinal analyses show that in a single year (2023-2024) there has been a rapid crescendo of data restrictions from web sources, rendering ~5%+ of all tokens in C4, or 28%+ of the most actively maintained, critical sources in C4, fully restricted from use. For Terms of Service crawling restrictions, a full 45% of C4 is now restricted. If respected or enforced, these restrictions are rapidly biasing the diversity, freshness, and scaling laws for general-purpose AI systems. We hope to illustrate the emerging crises in data consent, for both developers and creators. The foreclosure of much of the open web will impact not only commercial AI, but also non-commercial AI and academic research.

==> multimodal-analysis/8-datasets-methodology.tex <==

\subsection{Datasets}

The final phase of the AI data ecosystem is represented by curated datasets.
We assemble nearly $5,000$ popular datasets across text, video, and speech generation tasks, and annotate them for information encompassing (web) sources, creators, languages, and licenses.
The protocol for sourcing these datasets involved appointing team leads, who manually reviewed relevant dataset survey papers \citep{}, as well as the relevant modality's conferences and workshops for any datasets that fall in the scopes defined below.
We focus on text, video, and speech due to their importance in new foundation model development, and exclude images for lack of expertise in this domain---we leave this for future work.
All datasets are described, linked, and attributed in \suppinfo{app:datasets}.

\paragraph{Modality: Text} Following pretraining, large language models are commonly \emph{post-trained}, using collections of labelled finetuning datasets, preference datasets, and multi-dialog conversations. 
General-purpose models benefit from multi-task training on hetergeneous collections that span a variety of linguistic, reasoning, and knowledge intensive tasks, involving question answering, coding, tool use, creativity, translation, and classification.
Following the scope introduced by the Data Provenance Collection \citep{longpre2023data}, we expand their $44$ collections (of $1858$ supervised text datasets) to $100$ collections of $4500$ datasets \todo{replace numbers}, prioritizing recent, popular publicly available HuggingFace datasets introduced between 2022 and April 2024 \sara{but would this mainly involve post-training instruction finetuned texts -- how do we map this back to provisions about underlying data as we seem to do in the introduction?}.

\sara{big picture question here -- I find it kind of confusing the text datasets described here feel like majority intruction finetuning -- but it feels like they are being backed up into pretraining sources? Isn't the very nature of the transformation to intruction tuning mean they are fundamentally different -- this is the point we made in the data provenance paper. i.e. it feels reasonable as a story to say we focus on pretraining datasets like commoncrawl and backup to the terms of service and robots.txt -- it feels a bit of a jump to try to map that to licenses of instruction finetuned datasets which are transformed involving manual labor. This just feels like a seperate treatment? Feel like an extension of data provenance 1 -- where the story here is different -- in my mind it was about the changing attitudes around how people give consent to their data that ends up in pretraining datasets that are open source and widely used.}


\paragraph{Modality: Speech}
To curate a representative sample of datasets for automatic speech recognition (ASR), we employed a series of strategies. First, we searched for the most widely used datasets. We did this first by relying on our prior knowledge of common datasets in the ASR literature (e.g. LibriSpeech~\cite{panayotov2015librispeech}), then searching for the most popular datasets on Hugging Face Datasets, and finally consulting lists in repositories of popular speech datasets, curated by practitioners. Then, we worked on expanding coverage by looking for well-documented datasets on the OpenSLR\footnote{\href{https://openslr.org/}{openslr.org}: Open Speech and Language Resources} platform, even if they were newer or less widely used. We expect this might reflect datasets that could be adopted more in the future. OpenSLR is a widely used platform in the speech community, dedicated to hosting resources for speech tasks. Finally, we worked on adding datasets related to low-resource languages, and other languages not well-covered by our initial searches. Speech recognition models are increasingly highly multilingual, and datasets serving different communities of builders and end-users around the world are a priority to make speech recognition technologies more inclusive.

In many cases, multiple versions of a dataset exist due to datasets being expanded or updated. In these scenarios, we used the release date from the initial version (since release dates for subsequent versions were not always clear), but used metadata from the most recently released version for which information was available to offer an overview of the current landscape of data. However, if the dataset versions could not be meaningfully aggregated (e.g. different licenses), or did not appear to be cumulatively designed (non-overlapping or otherwise semantically disjoint data), we maintained separate records. We kept only datasets primarily intended for ASR. For example, if a dataset was primarily intended for text-to-speech or speaker recognition, we did not keep it even if it could conceivably be repurposed for ASR. When computing hours, we excluded any hours without supervisory transcripts/scripts (unlabeled data), but kept hours with ``weak supervision'' (e.g. model-generated transcripts from speech audio). We recognize the difficulty in comprehensively covering all relevant datasets. We aimed to collect a holistic and representative set with enough metadata available to extract insights about the current state of speech recognition data.

\paragraph{Modality: Video} Video Generation from language has emerged as an important task for new multimodal foundation models [Sora, cite others]. 
However, the number of publicly available datasets designed for text-to-video generation are limited (we found 15). 
The video understanding and generation community does however use a range of labelled datasets for related purposes \sara{do we have support for this? Just a note that this again seems to pose the issue that these are transformed datasets for the purposes of ml and so not clear how we can trace back to pretraining? I guess a wider question is since this feels jumpy -- is our focus pretraining scrapped from the web or labelled datasets created expressly for machine learning purposes? It feels muddled right now.}.
Therefore, to capture a wider representation of the video dataset ecosystem we have tailored our audit scope to include tasks that can be refactored for generation purposes.
This includes Video Captioning, Video Question Answering, Video Summarization, and Video Language understanding tasks. 
We have also included datasets for other popular tasks in the video community such as Action Recognition, Understanding, Egocentric View and Segmentation, Video Classification, Temporal Localization, and Group Activity Recognition. 
Our final collection includes 97 video datasets spanning the 13 most popular video tasks (based on citations and CVPR workshops) from 2009-2024.
We believe that our collection is a wide representative sample of datasets that could be used to generate videos in the future.  


==> multimodal-analysis/88-datasets.tex <==
\section{Auditing Datasets: Text, Speech \& Video}

\subsection{Speech}
\todo{Nikhil, Manuel}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/speech/speech_categories-years.png}
    \caption{Distribution of creator categories over time. Earlier datasets in our set were primarily contributed by academic creators, while recent datasets have more diversified creators including industry, nonprofit, and independent researchers.}
    \label{fig:speech_categories-years}
\end{figure}

Automatic Speech Recognition (ASR) has been an early adopter of data-driven modeling techniques, from Markov Models in the 1980s~\cite{bahl1983maximum, baker1975dragon, rabiner1989tutorial} to deep neural networks in the 2000s~\cite{hinton2012deep}. More recently, models have made tremendous strides in multilingualism, speaker independence, and robustness to noise, ambiguity, and environmental variation, all owing in large part to enormous, private datasets~\cite{radford2023robust, ramirez2024anatomy, zhang2024conformer}. This coincides with an increase in the proportion of industry dataset contributions (e.g. see Fig.~\ref{fig:speech_categories-years}), however the largest-scale of these remain relatively obscure to the public. The success of this commercial enterprise has motivated open replication efforts, to bring the benefits of high-quality ASR to a broader community~\cite{li2023yodas, peng2023reproducing}. However, canonical speech datasets are orders of magnitude smaller than those needed for state-of-the-art models, which extend into the hundreds of thousands and even millions of hours. Consequently, researchers have recently turned to sources like YouTube to obtain scalable data, which introduces new challenges in determining ownership and usage rights in addition to obscuring provenance information (e.g. information about the sample of speakers included, and their representativeness of the population of use).

\paragraph{Datasets Overview}
We survey datasets released from 1990 to 2024, coming from a total of 124 creators and 29 countries in academia, industry labs and corporations, nonprofits, governmental sources, and even independent researchers. They total over 700k hours with a median size of 332 hours and a mean of 8,164, suggesting that a few datasets contribute a large quantity of the hours (Gini coefficient $G=0.92$). These datasets cover more than 200 languages with 65 of them being monolingual, and the remainder ranging from 2 up to 149.

\paragraph{Licenses and Data Sources}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/speech/speech_sourcecategories-licenses.png}
    \caption{License type distributions for different source categories. Of note is that Internet Video-based datasets are largely licensed permissively, despite having potential copyright and terms of service implications. Conversely, TED Talk-based datasets inherit a more restrictive license. Licenses for categories like Crowd-Sourcing and Human Participants are often more at the dataset contributors' discretion, since they aren't typically aggregated from sources with licensing implications.}
    \label{fig:speech_sourcecategories-licenses}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/speech/speech_license-source.png}
    \caption{License type distributions, showing the specific case where datasets are taken (in whole or part) from YouTube, a platform with user-generated content and terms of service considerations: \textbf{(top)} by dataset count and \textbf{(bottom)} by hours of data. By count, it appears a few permissively licensed datasets are YouTube-based. However, by hours, it's clear that these datasets constitute a majority of the hours of speech recognition data made available for commercial use. This calls into question the viability of depending on such data, e.g. under the fair use exception.}
    \label{fig:speech_license-source}
\end{figure}

In our sample of speech datasets, 51 (54\%) were marked for commercial use, 21 (33\%) for non-commercial/academic use (including custom licenses), and 13 (14\%) were unspecified (including those which require inquiries for license information). However, 5 (10\%) out of 51 of the permissively-licensed datasets, accounting for 69\% of the total hours of speech permissively licensed, come from datasets which use YouTube (in part or fully), as we show in Fig.~\ref{fig:speech_license-source}. For this data, determining commercial usability is challenging and, for example, may be subject to fair use interpretation. Datasets may also sample permissively-licensed source videos, as with YODAS~\cite{li2023yodas}. Additionally, we often have more fine-grained provenance information for datasets drawing on conventional methods (e.g. crowd-sourcing and human participants), such as the number of speakers represented in the data, the topics spoken about, and, in some cases, overlap with other datasets (e.g. for those derived from other existing datasets).

\paragraph{Shifts in Data Sources}
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/speech/speech_sourcecategories-cumulativehours.png}
    \caption{Cumulative hours (symlog-scaled) of data from different sources over time. Internet Video contributions only emerged recently, and immediately became the largest data source due to scalability.}
    \label{fig:speech_sourcecategories-cumulativehours}
\end{figure}

Aggregating directly from sources such as YouTube makes it challenging to characterize such details, and thereby potentially challenging to understand the limits of the data as it applies to real-world end-user populations. However, over time we observe shifts in source categories, largely tending towards using such resources (see Fig.~\ref{fig:speech_sourcecategories-cumulativehours}). For example, calling platforms were an integral part of earlier speech datasets, but are not seen much recently. The proportion of datasets relying on human participants has reduced, though there remain some of these. By contrast, crowd-sourcing has steadily increased over time. Additionally, data from internet video sources like YouTube appear more in recent years. This data source emerged recently, and quickly ascended to become the most popular category (in hours). The increase in tapping internet video sources is likely due to their scalability and the demands of modern models and training regimes. This could also include the rise of self-supervised pre-training from unlabeled data before supervised training.

\paragraph{Linguistic Diversity and Representation}
Despite our best efforts to obtain wide language coverage in represented datasets, there remains a fair amount of inequality between languages. The Gini coefficient of hours in datasets which represent different languages, where we divide hours across languages for any multilingual datasets, is $G=0.52$, with Germanic and Indo-European family languages the most represented.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/speech/speech_languagefamilies-licenses.png}
    \caption{License types by datasets with different language families represented, showing a relatively stable distribution.}
    \label{fig:speech_languagefamilies-licenses}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/speech/speech_languagefamilies-sources.png}
    \caption{Source distributions by datasets with different language families represented, showing a relatively stable distribution.}
    \label{fig:speech_languagefamilies-sources}
\end{figure}

We observe that license types are relatively stable across language families (shown in Fig.~\ref{fig:speech_languagefamilies-licenses}), with Afroasiatic language-containing datasets having the lowest rate of permissive licenses (7/14, 50\%) associated with them, and Uralic the highest (4/5, 80\%). Source categories are also largely stable across language families (shown in Fig.~\ref{fig:speech_languagefamilies-sources}); Internet Video and Crowd-Sourcing appear consistently across them, and Human Participants and Audiobooks also appear in most. It’s important to note that we only have an indirect signal of this; we look at both sources and languages at the dataset level, not accounting for the precise distribution of source-language combinations within datasets since these are challenging to obtain.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/speech/speech_languages-giniyears.png}
    \caption{Gini coefficient for cumulative hours by represented languages over time. We observe a decrease (more equality) in recent years. It's important to note this doesn't reflect the precise proportions of different languages within such datasets, which is important for a more accurate view.}
    \label{fig:speech_languages-giniyears}
\end{figure}

We also look at the shift over time in terms of languages represented. Even without precise language compositions for different datasets, we can get a broad sense of representation considering that the majority of datasets we survey are monolingual. To look at the trend here, we take the cumulative sum of hours by language over time and compute the Gini coefficient within each year’s (cumulatively available) hours by language, concluding with the current Gini coefficient presented earlier, across all the data. This is given in Fig.~\ref{fig:speech_languages-giniyears} and shows recent large-scale dataset contributions have lowered this coefficient over time. This suggests that datasets are not only growing in size, but are also distributed across languages more, which could improve linguistic representation for speech recognition. However, it's important to note that because we do not know the precise proportions of languages represented within such datasets, we can only see that they are represented. Determining how well they are represented (e.g. how many hours in each dataset come from each constituent language) is an important next step in assessing language representation.

In summary, the distribution of and changes in speech recognition datasets highlight a tension between the rapid progress enabled by large-scale found data and the need for careful curation and documentation to ensure responsible development of the technology. The field's increasing reliance on sources like YouTube has allowed models to reach unprecedented capabilities, but obscures information about licensing, representation, and potential data biases. While this has enabled promising trends towards greater linguistic diversity, resource inequality between languages remains stark. Grappling with these sociotechnical considerations will be crucial to democratize the benefits of speech technology.

\tldr{Sharply summarize the state of public speech-to-text datasets.}

\todo{Summary table for Speech-to-Text Datasets: name, sizes, creators, popularity, languages, sources, license?, ++what else}

\tldr{How are licenses/terms/legal ambiguities distributed?}

\tldr{How are sources distributed?}

\tldr{How are creators distributed?}

\subsection{Video}

% describe video-specific stuff here - 
% what is in the video datasets/what do you wanna say about the analysis of the video datasets? 
% Most of the current datasets in the video domain were predominantly designed for action recognition task. The current research trends are shifting towards more sophisticated and fine-grained tasks like video generation. 
% As the field moves towards text-to-video generation, it is likely to encounter issues similar to those faced by large language models (LLMs). Many of the datasets being repurposed for these new tasks do not have clear licensing, which creates legal and ethical challenges. Additionally, the sources of these datasets are often YouTube or general web, where the ownership and rights to the training data are ambiguous. The concept of fair use, already a gray area in text generation, becomes even more nebulous when applied to generated video content.
% Out of the video datasets available, the largest percentage (41\%) is dedicated to video classification and action recognition. In contrast, video captioning datasets only make up 17\% of the most common datasets. Furthermore, a substantial portion of these datasets (38.5\%) have unspecified licenses, adding another layer of complexity to their use. Additionally, 32\% of these datasets come from YouTube and 15\% from movies, both of which typically do not offer robust licensing support. This situation underscores the need for clearer guidelines and better-designed datasets that can address the evolving needs of video-language research and ensure legal and ethical compliance.

The current state of video datasets reflects a rapidly evolving landscape, with a growing emphasis on supporting more complex and diverse tasks beyond simple action recognition. Among the audited video datasets, a considerable portion (41\%) is dedicated to video classification (12\%) and action recognition (29\%). Video generation tasks using video and language datasets only constitute 15\% of the most common datasets. However, other video tasks such as video captioning (17\%), summarization (3\%), and Q\&A (4\%) also contain video-text pairs that can be used for the video generation task. 

\paragraph{License Distribution.} However, progress is accompanied by significant challenges, particularly regarding dataset licensing and composition. Among the available video datasets, a substantial 38.5\% have unspecified licenses, adding another layer of complexity to their use. Several incredibly popular datasets in the video community such as MovieQA \cite{tapaswiMovieQAUnderstandingStories2016} (765 citations), MovieGraphs \cite{vicolMovieGraphsUnderstandingHumanCentric2018}  (146 citations), and, most notably, WebVid \cite{bainFrozenTimeJoint2022} (719 citations) have all been taken down due to cease and desist letters. In addition, 39\% of the video datasets have a Non-Commercial/Academic Licence. We refer our reader to Fig.~\ref{fig:license_use_by_modality}. 

\paragraph{Source Distribution.} The sources of video datasets are heavily skewed towards user-generated content platforms, with 33\% coming from YouTube, 20\% from human participants, and 15\% from movies. While these sources offer vast amounts of diverse and engaging video content, they also present challenges in terms of licensing and attribution. YouTube's terms of service, for example, place strict limits on the use of videos for training machine learning models, while movies often involve complex rights negotiations with multiple stakeholders. \textbf{citation/course to back this?} We refer our reader to Fig.(Fig.~\ref{fig:source_categories_by_modality}). 

\paragraph{Creator Distribution.} The creator distribution for Video skews heavily towards Academic institutions (68\%) which makes sense as the majority of the video research has been done in Academic institutions or Industry Research Labs with the majority of Academic and Research licences (Fig.~\ref{fig:source_categories_by_modality}). %However, as Video Generation becomes more mainstream and commercial, we anticipate more industry creators. 
However, as Video Generation becomes more mainstream and commercial, we anticipate more industry creators with commercial data sources and licenses. % add how many are from Europe/Asia & North America. write the names of those universities idk

\textbf{Conclusions \& Discussions.} As the field progresses toward text-to-video generation, it will likely encounter issues similar to those faced by large language models (LLMs). First, many datasets lack clear licensing, creating legal and ethical challenges (Fig.~\ref{fig:license_use_by_modality}). Second, the sources of these datasets are often YouTube or the general web, where the ownership and rights to the training data are ambiguous (Fig.~\ref{fig:source_categories_by_modality}). We anticipate that fair use, already a gray area in text generation, will become even more nebulous when applied to commercial generated video content.

% \todo{Kush, Joanna}
% \tldr{Sharply summarize the state of public text-to-video datasets: name, sizes, creators, popularity, sources, license?, ++what else}
% \todo{Summary table for Text-to-Video Datasets}
% \tldr{How are licenses/terms/legal ambiguities distributed?}
% \tldr{How are sources distributed?}
% \tldr{How are creators distributed?}

\subsection{Comparing Modalities}
% \todo{Ahmad}

\tldr{Plot: How do legal restrictions compare across text, video, speech?}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/multimodal/license_use_by_modality.png}
    \caption{License use by modality, grouped into either Non-Commercial/Academic, Unspecified, or Commercial use. The video modality has a much lower proportion of permissively licensed datasets than text or speech. Speech has the highest proportion of commercially usable datasets. Text and video also have higher proportions of unspecified licenses, making determining permissiveness more challenging.}
    \label{fig:license_use_by_modality}
\end{figure}

\tldr{Plot: How does the distribution of creators (by academia/startup/industry, and by geography) compare across text, video, speech?}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/multimodal/creator_categories_by_modality.png}
    \caption{Creator categories by modality. Overall, video has the highest proportion of Academic contributions, with speech having the lowest. Speech has a higher proportion of corporate, startup, and government contributions than both other modalities, but the lowest from industry research labs. Across all modalities, academia contributes the most datasets by a large margin.}
    \label{fig:creator_categories_by_modality}
\end{figure}

\tldr{Plot: How do data sources (machine/web/etc) compare across text, video, speech?}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/multimodal/source_categories_by_modality.png}
    \caption{Data sources, grouped into higher-level categories. Source distributions vary widely between modalities. For example, speech datasets rely more on human participants and crowd-sourcing than video and text. All datasets rely on cultural and entertainment sources such as books (text), audiobooks (speech), and movies (video). Speech and especially video rely more on social media and user-generated content, such as YouTube videos (and corresponding audio tracks). The \textit{Other} category includes sources like code (text), podcasts (speech), and the weather channel (video).}
    \label{fig:source_categories_by_modality}
\end{figure}

==> multimodal-analysis/legal_discussion.tex <==
\section{Legal Discussion}
\sara{this section feels a bit speculative, particularly for a neurips paper. This is probably a valid question for the authors about the degree to which interpretation of active case law is within our purview.}
Pretraining data provenance matters from at least three legal perspectives.
First, using pretraining data to develop AI models may violate the copyright of the underlying data even before any outputs are generated~\cite{epstein2023art}. % add more cites
In the U.S., this assessment depends in part on the degree to which the trained model competes with the creator of the underlying data.
We find that ...
While it may be more likely for pretraining data to be covered by fair use than finetuning data~\cite{mahari2023comment}, this is definitely not always the case and subject to active litigation.
Second, even if training the model does not violate copyright, generating a specific output may violate the copyright of some piece of the training data.
Both the users and providers of these systems may be engaging in direct copyright infringement, while those further up the supply chain may be indirectly liable~\cite{yew2024break}.
Data provenance is critical in these situations since copyright infringement needs to be assessed on a case-by-case basis. 
Robust data lineage may also help developers generate safeguards to avoid this type of infringement in the first place.
Third, data provenance is necessary for assessing data quality and robustness, which is increasingly required by AI regulation like the EU's AI Act.

==> sections/999-checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors:
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The abstract and introduction accurately describe our core contributions.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitations of our work, and assumptions of our empirical methods throughout the work.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} We discuss in Section \ref{sec:discussion} the implications of the findings of our work.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
        \answerYes{We have read the ethics review guidelines and made sure our paper conforms to them.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{No formal results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{No formal results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{No model training experiments, but our analysis code and data are available as described in the manuscript.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{No model training experiments.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{No model training experiments.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{No model training experiments.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We have cited the underlying datasets which were the subject of this audit study in our supplementary material, available as described in the manuscript. There are too many datasets to include all of them in this manuscript.}
  \item Did you mention the license of the assets?
    \answerYes{The supplementary material includes tables laying out the licenses and other conditions attached to these datasets.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Our analysis code and metadata are available as described in the manuscript.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All datasets we audit here are already publicly available for academic use.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{This is included in Section \ref{sec:methodology}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
        \answerYes{This is included in Appendix \ref{app:manual-annotation}.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{This is included in Appendix \ref{app:manual-annotation}.}
\end{enumerate}

\end{enumerate}

==> tables/attributes.tex <==
\begin{table*}[t!]
\centering
% \footnotesize
\renewcommand{\arraystretch}{1.5}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{p{3cm} | p{14cm} | p{0.5cm}p{0.5cm}p{0.5cm}}
\toprule
\textsc{Attribute} & \textsc{Details} & \textsc{T} & \textsc{V} & \textsc{S}  \\
\midrule

\textbf{Aggregator Links} & Instances of the dataset on GitHub, HuggingFace, Papers with Code, ArXiv, and Semantic Scholar are manually linked. This allows artifact, usage, and licensing metadata to be cross-referenced.  & \greencheck & \greencheck & \greencheck \\ \rowcolor[gray]{0.9}
\textbf{Sources} & The original sources from which the data was collected. This includes websites or databases, human annotation, and model-generated content, wherever disclosed.  & \greencheck & \greencheck & \greencheck \\
\textbf{Licenses} & The dataset licenses and license URLs found on associated GitHub, HuggingFace, website, and academic paper pages. We also use \citet{longpre2023data} guidelines to classify licenses by use type (non-commercial, unspecified, all uses permitted), attribution, and copyleft restrictions.  & \greencheck & \greencheck & \greencheck \\ \rowcolor[gray]{0.9}
\textbf{Creators} & The organizations attributed with curating the dataset (not the underlying data). These organizations are categorized by country and by industry vs academia. & \greencheck & \greencheck & \greencheck \\
\textbf{Tasks} & The specific tasks associated with the supervised datasets. & \greencheck & \greencheck & \greencheck \\ \rowcolor[gray]{0.9}
\textbf{Size Metrics} & The size of the dataset, measured in dialog turns and tokens for text, the number of videos, or the number of hours and speakers for speech.  & \greencheck & \greencheck & \greencheck \\
\midrule
\textbf{Languages} & The languages represented in the text of speech, and their associated language families.  & \greencheck &  & \greencheck \\

\bottomrule
\end{tabular}
\end{adjustbox}
% \captionsetup{justification=centering}
\caption{The \textbf{list of dataset attributes}, their collection process, and the modalities they were collected for. All attributes are manually collected. Annotation guidelines are available in \cref{app:attribute-annotation}.}
\label{tab:attributes}
\vspace{-2mm}
\end{table*}



==> tables/collections-audio.tex <==
\setlength{\tabcolsep}{1.9pt}
\definecolor{colorTIMITPropertyCounts_Hr}{RGB}{244,229,189}
\definecolor{colorSwitchboardPropertyCounts_Hr}{RGB}{245,241,232}
\definecolor{colorAfricanAcc.FrenchPropertyCounts_Hr}{RGB}{245,235,206}
\definecolor{colorCSJPropertyCounts_Hr}{RGB}{245,244,242}
\definecolor{colorFisherPropertyCounts_Hr}{RGB}{236,243,242}
\definecolor{colorCSLU22Langs.PropertyCounts_Hr}{RGB}{245,238,220}
\definecolor{colorAMIPropertyCounts_Hr}{RGB}{245,239,222}
\definecolor{colorCSLU1.2PropertyCounts_Hr}{RGB}{245,235,208}
\definecolor{colorALLSSTARPropertyCounts_Hr}{RGB}{245,238,220}
\definecolor{colorTED-LIUM3PropertyCounts_Hr}{RGB}{245,243,238}
\definecolor{colorNSTNorwegianPropertyCounts_Hr}{RGB}{245,243,240}
\definecolor{colorNSTDanishPropertyCounts_Hr}{RGB}{245,243,240}
\definecolor{colorNSTSwedishPropertyCounts_Hr}{RGB}{245,242,234}
\definecolor{colorVystadialPropertyCounts_Hr}{RGB}{245,237,216}
\definecolor{colorTHCHS-30PropertyCounts_Hr}{RGB}{245,236,212}
\definecolor{colorLibriSpeechPropertyCounts_Hr}{RGB}{244,244,244}
\definecolor{colorTHUYG-20PropertyCounts_Hr}{RGB}{245,235,206}
\definecolor{colorVCTKPropertyCounts_Hr}{RGB}{245,237,214}
\definecolor{colorSpokenWikipediaPropertyCounts_Hr}{RGB}{244,244,244}
\definecolor{colorAISHELL-1PropertyCounts_Hr}{RGB}{245,243,240}
\definecolor{colorLJSpeechPropertyCounts_Hr}{RGB}{245,235,208}
\definecolor{colorClarinPLPropertyCounts_Hr}{RGB}{245,237,216}
\definecolor{colorAISHELL-2PropertyCounts_Hr}{RGB}{244,244,244}
\definecolor{colorRegionalAf.Am.Lang.PropertyCounts_Hr}{RGB}{245,240,228}
\definecolor{colorCrowdSourcedSpeechPropertyCounts_Hr}{RGB}{242,244,244}
\definecolor{colorZeroth-KoreanPropertyCounts_Hr}{RGB}{245,239,222}
\definecolor{colorRTVEPropertyCounts_Hr}{RGB}{245,244,242}
\definecolor{colorOpenSTTPropertyCounts_Hr}{RGB}{215,237,234}
\definecolor{colorMuST-CPropertyCounts_Hr}{RGB}{231,241,240}
\definecolor{colorM-AILABSPropertyCounts_Hr}{RGB}{244,244,244}
\definecolor{colorMAGICDATAPropertyCounts_Hr}{RGB}{245,244,244}
\definecolor{colorCommonVoice17PropertyCounts_Hr}{RGB}{211,237,233}
\definecolor{colorCoNASEPropertyCounts_Hr}{RGB}{193,231,226}
\definecolor{colorNigerianEnglishPropertyCounts_Hr}{RGB}{245,230,192}
\definecolor{colorNorwegianParl.SpeechPropertyCounts_Hr}{RGB}{245,240,226}
\definecolor{color120hSpanishSpeechPropertyCounts_Hr}{RGB}{245,239,224}
\definecolor{colorDiDiSpeechPropertyCounts_Hr}{RGB}{245,244,244}
\definecolor{colorCzechParliamentPropertyCounts_Hr}{RGB}{245,243,238}
\definecolor{colorCoVoST-2PropertyCounts_Hr}{RGB}{233,242,240}
\definecolor{colorKSCPropertyCounts_Hr}{RGB}{245,242,234}
\definecolor{colorBasq.,Cat.andGal.PropertyCounts_Hr}{RGB}{245,236,210}
\definecolor{colorKsponSpeechPropertyCounts_Hr}{RGB}{244,244,244}
\definecolor{colorSamromurPropertyCounts_Hr}{RGB}{245,240,226}
\definecolor{colorMultiling.LibriSpeechPropertyCounts_Hr}{RGB}{206,235,231}
\definecolor{colorMaSSPropertyCounts_Hr}{RGB}{245,240,228}
\definecolor{colorFTSPEECHPropertyCounts_Hr}{RGB}{236,243,242}
\definecolor{colorEng.Acc.inBrit.IslesPropertyCounts_Hr}{RGB}{245,236,210}
\definecolor{colorHighlandPueblaNahuatlPropertyCounts_Hr}{RGB}{245,240,226}
\definecolor{colorQASRPropertyCounts_Hr}{RGB}{236,243,242}
\definecolor{colorMultiling.TEDxPropertyCounts_Hr}{RGB}{245,244,244}
\definecolor{colorMinds14PropertyCounts_Hr}{RGB}{245,235,208}
\definecolor{colorGolosPropertyCounts_Hr}{RGB}{242,244,244}
\definecolor{colorMASCPropertyCounts_Hr}{RGB}{242,244,244}
\definecolor{colorLaboroTVSpeechPropertyCounts_Hr}{RGB}{236,243,242}
\definecolor{colorKeSpeechPropertyCounts_Hr}{RGB}{238,243,242}
\definecolor{colorJTUBESPEECHPropertyCounts_Hr}{RGB}{240,243,243}
\definecolor{colorGigaSpeechPropertyCounts_Hr}{RGB}{222,239,237}
\definecolor{colorVoxPopuliPropertyCounts_Hr}{RGB}{238,243,242}
\definecolor{colorSPGISpeechPropertyCounts_Hr}{RGB}{227,240,239}
\definecolor{colorWestAfr.RadioPropertyCounts_Hr}{RGB}{245,240,226}
\definecolor{colorAISHELL-4PropertyCounts_Hr}{RGB}{245,239,224}
\definecolor{colorWestAfr.Virt.Asst.PropertyCounts_Hr}{RGB}{239,221,175}
\definecolor{colorMediaSpeechPropertyCounts_Hr}{RGB}{245,236,212}
\definecolor{colorPeople'sSpeechPropertyCounts_Hr}{RGB}{211,237,233}
\definecolor{color1111HoursHindiPropertyCounts_Hr}{RGB}{245,239,224}
\definecolor{colorShrutilipiPropertyCounts_Hr}{RGB}{226,240,238}
\definecolor{colorWenetSpeechPropertyCounts_Hr}{RGB}{222,239,237}
\definecolor{colorSamromurChildrenPropertyCounts_Hr}{RGB}{245,240,226}
\definecolor{colorSDS-200PropertyCounts_Hr}{RGB}{245,241,230}
\definecolor{coloraidatatangPropertyCounts_Hr}{RGB}{245,241,230}
\definecolor{colorFleursPropertyCounts_Hr}{RGB}{240,243,243}
\definecolor{colorOLKAVSPropertyCounts_Hr}{RGB}{242,244,244}
\definecolor{colorNorwegianParl.PropertyCounts_Hr}{RGB}{245,240,226}
\definecolor{colorMagicData-RAMCPropertyCounts_Hr}{RGB}{245,240,228}
\definecolor{colorKathbathPropertyCounts_Hr}{RGB}{238,243,242}
\definecolor{colorHebrewKanPropertyCounts_Hr}{RGB}{245,232,196}
\definecolor{colorHebrewCourseraPropertyCounts_Hr}{RGB}{245,236,212}
\definecolor{colorBloomSpeechPropertyCounts_Hr}{RGB}{245,243,238}
\definecolor{colorEnglish-VietnamesePropertyCounts_Hr}{RGB}{245,243,240}
\definecolor{colorEarnings-22PropertyCounts_Hr}{RGB}{245,239,224}
\definecolor{colorYODASPropertyCounts_Hr}{RGB}{179,226,219}
\definecolor{colorAFRISPEECH-200PropertyCounts_Hr}{RGB}{245,241,230}
\definecolor{colorAaltoFinnishParl.PropertyCounts_Hr}{RGB}{233,242,240}
\definecolor{colorReazonSpeechPropertyCounts_Hr}{RGB}{209,236,232}
\definecolor{colorEdAccPropertyCounts_Hr}{RGB}{245,236,212}
\definecolor{colorRixVoxPropertyCounts_Hr}{RGB}{227,240,239}
\definecolor{colorJapaneseAnimeSpeechPropertyCounts_Hr}{RGB}{245,239,224}
\definecolor{colorSnowMountainPropertyCounts_Hr}{RGB}{245,241,232}
\definecolor{colorSamromurMilljonPropertyCounts_Hr}{RGB}{244,244,244}
\definecolor{colorBud500PropertyCounts_Hr}{RGB}{245,243,240}
\definecolor{colorVibraVoxPropertyCounts_Hr}{RGB}{245,234,204}
\definecolor{colorM2ASRPropertyCounts_Hr}{RGB}{245,243,238}
\definecolor{colorTIMITPropertyCounts_Spkr}{RGB}{215,237,234}
\definecolor{colorSwitchboardPropertyCounts_Spkr}{RGB}{215,237,234}
\definecolor{colorAfricanAcc.FrenchPropertyCounts_Spkr}{RGB}{218,238,235}
\definecolor{colorCSJPropertyCounts_Spkr}{RGB}{211,237,233}
\definecolor{colorFisherPropertyCounts_Spkr}{RGB}{202,234,230}
\definecolor{colorCSLU22Langs.PropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorAMIPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorCSLU1.2PropertyCounts_Spkr}{RGB}{206,235,231}
\definecolor{colorALLSSTARPropertyCounts_Spkr}{RGB}{220,239,236}
\definecolor{colorTED-LIUM3PropertyCounts_Spkr}{RGB}{209,236,232}
\definecolor{colorNSTNorwegianPropertyCounts_Spkr}{RGB}{213,237,234}
\definecolor{colorNSTDanishPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorNSTSwedishPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorVystadialPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorTHCHS-30PropertyCounts_Spkr}{RGB}{226,240,238}
\definecolor{colorLibriSpeechPropertyCounts_Spkr}{RGB}{208,236,232}
\definecolor{colorTHUYG-20PropertyCounts_Spkr}{RGB}{217,238,235}
\definecolor{colorVCTKPropertyCounts_Spkr}{RGB}{222,239,237}
\definecolor{colorSpokenWikipediaPropertyCounts_Spkr}{RGB}{213,237,234}
\definecolor{colorAISHELL-1PropertyCounts_Spkr}{RGB}{217,238,235}
\definecolor{colorLJSpeechPropertyCounts_Spkr}{RGB}{242,244,244}
\definecolor{colorClarinPLPropertyCounts_Spkr}{RGB}{217,238,235}
\definecolor{colorAISHELL-2PropertyCounts_Spkr}{RGB}{209,236,232}
\definecolor{colorRegionalAf.Am.Lang.PropertyCounts_Spkr}{RGB}{218,238,235}
\definecolor{colorCrowdSourcedSpeechPropertyCounts_Spkr}{RGB}{208,236,232}
\definecolor{colorZeroth-KoreanPropertyCounts_Spkr}{RGB}{220,239,236}
\definecolor{colorRTVEPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorOpenSTTPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorMuST-CPropertyCounts_Spkr}{RGB}{209,236,232}
\definecolor{colorM-AILABSPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorMAGICDATAPropertyCounts_Spkr}{RGB}{211,237,233}
\definecolor{colorCommonVoice17PropertyCounts_Spkr}{RGB}{179,226,219}
\definecolor{colorCoNASEPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorNigerianEnglishPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorNorwegianParl.SpeechPropertyCounts_Spkr}{RGB}{217,238,235}
\definecolor{color120hSpanishSpeechPropertyCounts_Spkr}{RGB}{229,241,239}
\definecolor{colorDiDiSpeechPropertyCounts_Spkr}{RGB}{204,235,230}
\definecolor{colorCzechParliamentPropertyCounts_Spkr}{RGB}{218,238,235}
\definecolor{colorCoVoST-2PropertyCounts_Spkr}{RGB}{190,230,224}
\definecolor{colorKSCPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorBasq.,Cat.andGal.PropertyCounts_Spkr}{RGB}{220,239,236}
\definecolor{colorKsponSpeechPropertyCounts_Spkr}{RGB}{209,236,232}
\definecolor{colorSamromurPropertyCounts_Spkr}{RGB}{202,234,230}
\definecolor{colorMultiling.LibriSpeechPropertyCounts_Spkr}{RGB}{204,235,230}
\definecolor{colorMaSSPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorFTSPEECHPropertyCounts_Spkr}{RGB}{217,238,235}
\definecolor{colorEng.Acc.inBrit.IslesPropertyCounts_Spkr}{RGB}{222,239,237}
\definecolor{colorHighlandPueblaNahuatlPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorQASRPropertyCounts_Spkr}{RGB}{202,234,230}
\definecolor{colorMultiling.TEDxPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorMinds14PropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorGolosPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorMASCPropertyCounts_Spkr}{RGB}{200,234,229}
\definecolor{colorLaboroTVSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorKeSpeechPropertyCounts_Spkr}{RGB}{199,234,229}
\definecolor{colorJTUBESPEECHPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorGigaSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorVoxPopuliPropertyCounts_Spkr}{RGB}{206,235,231}
\definecolor{colorSPGISpeechPropertyCounts_Spkr}{RGB}{193,231,226}
\definecolor{colorWestAfr.RadioPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorAISHELL-4PropertyCounts_Spkr}{RGB}{224,240,237}
\definecolor{colorWestAfr.Virt.Asst.PropertyCounts_Spkr}{RGB}{226,240,238}
\definecolor{colorMediaSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorPeople'sSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{color1111HoursHindiPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorShrutilipiPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorWenetSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorSamromurChildrenPropertyCounts_Spkr}{RGB}{208,236,232}
\definecolor{colorSDS-200PropertyCounts_Spkr}{RGB}{206,235,231}
\definecolor{coloraidatatangPropertyCounts_Spkr}{RGB}{215,237,234}
\definecolor{colorFleursPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorOLKAVSPropertyCounts_Spkr}{RGB}{211,237,233}
\definecolor{colorNorwegianParl.PropertyCounts_Spkr}{RGB}{218,238,235}
\definecolor{colorMagicData-RAMCPropertyCounts_Spkr}{RGB}{213,237,234}
\definecolor{colorKathbathPropertyCounts_Spkr}{RGB}{211,237,233}
\definecolor{colorHebrewKanPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorHebrewCourseraPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorBloomSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorEnglish-VietnamesePropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorEarnings-22PropertyCounts_Spkr}{RGB}{222,239,237}
\definecolor{colorYODASPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorAFRISPEECH-200PropertyCounts_Spkr}{RGB}{208,236,232}
\definecolor{colorAaltoFinnishParl.PropertyCounts_Spkr}{RGB}{215,237,234}
\definecolor{colorReazonSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorEdAccPropertyCounts_Spkr}{RGB}{222,239,237}
\definecolor{colorRixVoxPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorJapaneseAnimeSpeechPropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorSnowMountainPropertyCounts_Spkr}{RGB}{231,241,240}
\definecolor{colorSamromurMilljonPropertyCounts_Spkr}{RGB}{200,234,229}
\definecolor{colorBud500PropertyCounts_Spkr}{RGB}{240,223,178}
\definecolor{colorVibraVoxPropertyCounts_Spkr}{RGB}{218,238,235}
\definecolor{colorM2ASRPropertyCounts_Spkr}{RGB}{215,237,234}
\definecolor{colorTIMITPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorSwitchboardPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorAfricanAcc.FrenchPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorCSJPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorFisherPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorCSLU22Langs.PropertyCounts_Lang}{RGB}{233,242,240}
\definecolor{colorAMIPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorCSLU1.2PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorALLSSTARPropertyCounts_Lang}{RGB}{226,240,238}
\definecolor{colorTED-LIUM3PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorNSTNorwegianPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorNSTDanishPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorNSTSwedishPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorVystadialPropertyCounts_Lang}{RGB}{245,233,198}
\definecolor{colorTHCHS-30PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorLibriSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorTHUYG-20PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorVCTKPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorSpokenWikipediaPropertyCounts_Lang}{RGB}{245,236,210}
\definecolor{colorAISHELL-1PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorLJSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorClarinPLPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorAISHELL-2PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorRegionalAf.Am.Lang.PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorCrowdSourcedSpeechPropertyCounts_Lang}{RGB}{245,239,222}
\definecolor{colorZeroth-KoreanPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorRTVEPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorOpenSTTPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorMuST-CPropertyCounts_Lang}{RGB}{238,243,242}
\definecolor{colorM-AILABSPropertyCounts_Lang}{RGB}{245,242,234}
\definecolor{colorMAGICDATAPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorCommonVoice17PropertyCounts_Lang}{RGB}{187,229,223}
\definecolor{colorCoNASEPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorNigerianEnglishPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorNorwegianParl.SpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{color120hSpanishSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorDiDiSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorCzechParliamentPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorCoVoST-2PropertyCounts_Lang}{RGB}{231,241,240}
\definecolor{colorKSCPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorBasq.,Cat.andGal.PropertyCounts_Lang}{RGB}{245,236,210}
\definecolor{colorKsponSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorSamromurPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorMultiling.LibriSpeechPropertyCounts_Lang}{RGB}{245,242,234}
\definecolor{colorMaSSPropertyCounts_Lang}{RGB}{245,242,234}
\definecolor{colorFTSPEECHPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorEng.Acc.inBrit.IslesPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorHighlandPueblaNahuatlPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorQASRPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorMultiling.TEDxPropertyCounts_Lang}{RGB}{245,243,238}
\definecolor{colorMinds14PropertyCounts_Lang}{RGB}{242,244,244}
\definecolor{colorGolosPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorMASCPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorLaboroTVSpeechPropertyCounts_Lang}{RGB}{245,233,198}
\definecolor{colorKeSpeechPropertyCounts_Lang}{RGB}{245,233,198}
\definecolor{colorJTUBESPEECHPropertyCounts_Lang}{RGB}{245,233,198}
\definecolor{colorGigaSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorVoxPopuliPropertyCounts_Lang}{RGB}{238,243,242}
\definecolor{colorSPGISpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorWestAfr.RadioPropertyCounts_Lang}{RGB}{245,243,240}
\definecolor{colorAISHELL-4PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorWestAfr.Virt.Asst.PropertyCounts_Lang}{RGB}{245,236,210}
\definecolor{colorMediaSpeechPropertyCounts_Lang}{RGB}{245,237,216}
\definecolor{colorPeople'sSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{color1111HoursHindiPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorShrutilipiPropertyCounts_Lang}{RGB}{245,244,244}
\definecolor{colorWenetSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorSamromurChildrenPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorSDS-200PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{coloraidatatangPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorFleursPropertyCounts_Lang}{RGB}{193,231,226}
\definecolor{colorOLKAVSPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorNorwegianParl.PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorMagicData-RAMCPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorKathbathPropertyCounts_Lang}{RGB}{245,244,244}
\definecolor{colorHebrewKanPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorHebrewCourseraPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorBloomSpeechPropertyCounts_Lang}{RGB}{209,236,232}
\definecolor{colorEnglish-VietnamesePropertyCounts_Lang}{RGB}{245,233,198}
\definecolor{colorEarnings-22PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorYODASPropertyCounts_Lang}{RGB}{179,226,219}
\definecolor{colorAFRISPEECH-200PropertyCounts_Lang}{RGB}{233,242,240}
\definecolor{colorAaltoFinnishParl.PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorReazonSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorEdAccPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorRixVoxPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorJapaneseAnimeSpeechPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorSnowMountainPropertyCounts_Lang}{RGB}{242,244,244}
\definecolor{colorSamromurMilljonPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorBud500PropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorVibraVoxPropertyCounts_Lang}{RGB}{240,223,178}
\definecolor{colorM2ASRPropertyCounts_Lang}{RGB}{245,237,216}
\definecolor{colorTIMITPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorSwitchboardPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorAfricanAcc.FrenchPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorCSJPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorFisherPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorCSLU22Langs.PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorAMIPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorCSLU1.2PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorALLSSTARPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorTED-LIUM3PropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorNSTNorwegianPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorNSTDanishPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorNSTSwedishPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorVystadialPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorTHCHS-30PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorLibriSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorTHUYG-20PropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorVCTKPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorSpokenWikipediaPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorAISHELL-1PropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorLJSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorClarinPLPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorAISHELL-2PropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorRegionalAf.Am.Lang.PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorCrowdSourcedSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorZeroth-KoreanPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorRTVEPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorOpenSTTPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorMuST-CPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorM-AILABSPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorMAGICDATAPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorCommonVoice17PropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorCoNASEPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorNigerianEnglishPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorNorwegianParl.SpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{color120hSpanishSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorDiDiSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorCzechParliamentPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorCoVoST-2PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorKSCPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorBasq.,Cat.andGal.PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorKsponSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorSamromurPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorMultiling.LibriSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorMaSSPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorFTSPEECHPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorEng.Acc.inBrit.IslesPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorHighlandPueblaNahuatlPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorQASRPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorMultiling.TEDxPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorMinds14PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorGolosPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorMASCPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorLaboroTVSpeechPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorKeSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorJTUBESPEECHPropertyCounts_Creat}{RGB}{242,244,244}
\definecolor{colorGigaSpeechPropertyCounts_Creat}{RGB}{206,235,231}
\definecolor{colorVoxPopuliPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorSPGISpeechPropertyCounts_Creat}{RGB}{242,244,244}
\definecolor{colorWestAfr.RadioPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorAISHELL-4PropertyCounts_Creat}{RGB}{242,244,244}
\definecolor{colorWestAfr.Virt.Asst.PropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorMediaSpeechPropertyCounts_Creat}{RGB}{231,241,240}
\definecolor{colorPeople'sSpeechPropertyCounts_Creat}{RGB}{217,238,235}
\definecolor{color1111HoursHindiPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorShrutilipiPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorWenetSpeechPropertyCounts_Creat}{RGB}{242,244,244}
\definecolor{colorSamromurChildrenPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorSDS-200PropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{coloraidatatangPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorFleursPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorOLKAVSPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorNorwegianParl.PropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorMagicData-RAMCPropertyCounts_Creat}{RGB}{242,244,244}
\definecolor{colorKathbathPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorHebrewKanPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorHebrewCourseraPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorBloomSpeechPropertyCounts_Creat}{RGB}{231,241,240}
\definecolor{colorEnglish-VietnamesePropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorEarnings-22PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorYODASPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorAFRISPEECH-200PropertyCounts_Creat}{RGB}{179,226,219}
\definecolor{colorAaltoFinnishParl.PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorReazonSpeechPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorEdAccPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorRixVoxPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorJapaneseAnimeSpeechPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorSnowMountainPropertyCounts_Creat}{RGB}{245,237,214}
\definecolor{colorSamromurMilljonPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorBud500PropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorVibraVoxPropertyCounts_Creat}{RGB}{240,223,178}
\definecolor{colorM2ASRPropertyCounts_Creat}{RGB}{245,242,234}
\definecolor{colorTIMITPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorSwitchboardPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorAfricanAcc.FrenchPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorCSJPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorFisherPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorCSLU22Langs.PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorAMIPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorCSLU1.2PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorALLSSTARPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorTED-LIUM3PropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorNSTNorwegianPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorNSTDanishPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorNSTSwedishPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorVystadialPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorTHCHS-30PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorLibriSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorTHUYG-20PropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorVCTKPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorSpokenWikipediaPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorAISHELL-1PropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorLJSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorClarinPLPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorAISHELL-2PropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorRegionalAf.Am.Lang.PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorCrowdSourcedSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorZeroth-KoreanPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorRTVEPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorOpenSTTPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorMuST-CPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorM-AILABSPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorMAGICDATAPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorCommonVoice17PropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorCoNASEPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorNigerianEnglishPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorNorwegianParl.SpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{color120hSpanishSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorDiDiSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorCzechParliamentPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorCoVoST-2PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorKSCPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorBasq.,Cat.andGal.PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorKsponSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorSamromurPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorMultiling.LibriSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorMaSSPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorFTSPEECHPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorEng.Acc.inBrit.IslesPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorHighlandPueblaNahuatlPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorQASRPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorMultiling.TEDxPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorMinds14PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorGolosPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorMASCPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorLaboroTVSpeechPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorKeSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorJTUBESPEECHPropertyCounts_Tasks}{RGB}{242,244,244}
\definecolor{colorGigaSpeechPropertyCounts_Tasks}{RGB}{206,235,231}
\definecolor{colorVoxPopuliPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorSPGISpeechPropertyCounts_Tasks}{RGB}{242,244,244}
\definecolor{colorWestAfr.RadioPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorAISHELL-4PropertyCounts_Tasks}{RGB}{242,244,244}
\definecolor{colorWestAfr.Virt.Asst.PropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorMediaSpeechPropertyCounts_Tasks}{RGB}{231,241,240}
\definecolor{colorPeople'sSpeechPropertyCounts_Tasks}{RGB}{217,238,235}
\definecolor{color1111HoursHindiPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorShrutilipiPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorWenetSpeechPropertyCounts_Tasks}{RGB}{242,244,244}
\definecolor{colorSamromurChildrenPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorSDS-200PropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{coloraidatatangPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorFleursPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorOLKAVSPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorNorwegianParl.PropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorMagicData-RAMCPropertyCounts_Tasks}{RGB}{242,244,244}
\definecolor{colorKathbathPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorHebrewKanPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorHebrewCourseraPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorBloomSpeechPropertyCounts_Tasks}{RGB}{231,241,240}
\definecolor{colorEnglish-VietnamesePropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorEarnings-22PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorYODASPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorAFRISPEECH-200PropertyCounts_Tasks}{RGB}{179,226,219}
\definecolor{colorAaltoFinnishParl.PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorReazonSpeechPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorEdAccPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorRixVoxPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorJapaneseAnimeSpeechPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorSnowMountainPropertyCounts_Tasks}{RGB}{245,237,214}
\definecolor{colorSamromurMilljonPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorBud500PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorVibraVoxPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorM2ASRPropertyCounts_Tasks}{RGB}{245,242,234}
\definecolor{colorTIMITPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorSwitchboardPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorAfricanAcc.FrenchPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorCSJPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorFisherPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorCSLU22Langs.PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorAMIPropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorCSLU1.2PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorALLSSTARPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorTED-LIUM3PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorNSTNorwegianPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorNSTDanishPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorNSTSwedishPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorVystadialPropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorTHCHS-30PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorLibriSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorTHUYG-20PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorVCTKPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorSpokenWikipediaPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorAISHELL-1PropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorLJSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorClarinPLPropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorAISHELL-2PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorRegionalAf.Am.Lang.PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorCrowdSourcedSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorZeroth-KoreanPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorRTVEPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorOpenSTTPropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorMuST-CPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorM-AILABSPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMAGICDATAPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorCommonVoice17PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorCoNASEPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorNigerianEnglishPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorNorwegianParl.SpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{color120hSpanishSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorDiDiSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorCzechParliamentPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorCoVoST-2PropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorKSCPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorBasq.,Cat.andGal.PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorKsponSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorSamromurPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMultiling.LibriSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMaSSPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorFTSPEECHPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorEng.Acc.inBrit.IslesPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorHighlandPueblaNahuatlPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorQASRPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMultiling.TEDxPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMinds14PropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorGolosPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMASCPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorLaboroTVSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorKeSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorJTUBESPEECHPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorGigaSpeechPropertyCounts_Src}{RGB}{245,243,238}
\definecolor{colorVoxPopuliPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorSPGISpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorWestAfr.RadioPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorAISHELL-4PropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorWestAfr.Virt.Asst.PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMediaSpeechPropertyCounts_Src}{RGB}{179,226,219}
\definecolor{colorPeople'sSpeechPropertyCounts_Src}{RGB}{245,237,216}
\definecolor{color1111HoursHindiPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorShrutilipiPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorWenetSpeechPropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorSamromurChildrenPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorSDS-200PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{coloraidatatangPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorFleursPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorOLKAVSPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorNorwegianParl.PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorMagicData-RAMCPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorKathbathPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorHebrewKanPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorHebrewCourseraPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorBloomSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorEnglish-VietnamesePropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorEarnings-22PropertyCounts_Src}{RGB}{245,243,238}
\definecolor{colorYODASPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorAFRISPEECH-200PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorAaltoFinnishParl.PropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorReazonSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorEdAccPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorRixVoxPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorJapaneseAnimeSpeechPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorSnowMountainPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorSamromurMilljonPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorBud500PropertyCounts_Src}{RGB}{245,237,216}
\definecolor{colorVibraVoxPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorM2ASRPropertyCounts_Src}{RGB}{240,223,178}
\definecolor{colorTIMITPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorSwitchboardPropertyCounts_Top}{RGB}{196,232,227}
\definecolor{colorAfricanAcc.FrenchPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorCSJPropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorFisherPropertyCounts_Top}{RGB}{213,237,234}
\definecolor{colorCSLU22Langs.PropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorAMIPropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorCSLU1.2PropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorALLSSTARPropertyCounts_Top}{RGB}{245,236,212}
\definecolor{colorTED-LIUM3PropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorNSTNorwegianPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorNSTDanishPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorNSTSwedishPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorVystadialPropertyCounts_Top}{RGB}{245,236,212}
\definecolor{colorTHCHS-30PropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorLibriSpeechPropertyCounts_Top}{RGB}{179,226,219}
\definecolor{colorTHUYG-20PropertyCounts_Top}{RGB}{245,236,212}
\definecolor{colorVCTKPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorSpokenWikipediaPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorAISHELL-1PropertyCounts_Top}{RGB}{244,244,244}
\definecolor{colorLJSpeechPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorClarinPLPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorAISHELL-2PropertyCounts_Top}{RGB}{245,243,238}
\definecolor{colorRegionalAf.Am.Lang.PropertyCounts_Top}{RGB}{245,243,238}
\definecolor{colorCrowdSourcedSpeechPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorZeroth-KoreanPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorRTVEPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorOpenSTTPropertyCounts_Top}{RGB}{245,241,230}
\definecolor{colorMuST-CPropertyCounts_Top}{RGB}{245,238,220}
\definecolor{colorM-AILABSPropertyCounts_Top}{RGB}{217,238,235}
\definecolor{colorMAGICDATAPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorCommonVoice17PropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorCoNASEPropertyCounts_Top}{RGB}{245,241,230}
\definecolor{colorNigerianEnglishPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorNorwegianParl.SpeechPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{color120hSpanishSpeechPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorDiDiSpeechPropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorCzechParliamentPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorCoVoST-2PropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorKSCPropertyCounts_Top}{RGB}{245,240,226}
\definecolor{colorBasq.,Cat.andGal.PropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorKsponSpeechPropertyCounts_Top}{RGB}{245,241,230}
\definecolor{colorSamromurPropertyCounts_Top}{RGB}{245,240,226}
\definecolor{colorMultiling.LibriSpeechPropertyCounts_Top}{RGB}{217,238,235}
\definecolor{colorMaSSPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorFTSPEECHPropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorEng.Acc.inBrit.IslesPropertyCounts_Top}{RGB}{245,238,220}
\definecolor{colorHighlandPueblaNahuatlPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorQASRPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorMultiling.TEDxPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorMinds14PropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorGolosPropertyCounts_Top}{RGB}{245,241,230}
\definecolor{colorMASCPropertyCounts_Top}{RGB}{235,242,241}
\definecolor{colorLaboroTVSpeechPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorKeSpeechPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorJTUBESPEECHPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorGigaSpeechPropertyCounts_Top}{RGB}{224,240,237}
\definecolor{colorVoxPopuliPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorSPGISpeechPropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorWestAfr.RadioPropertyCounts_Top}{RGB}{245,236,212}
\definecolor{colorAISHELL-4PropertyCounts_Top}{RGB}{245,241,230}
\definecolor{colorWestAfr.Virt.Asst.PropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorMediaSpeechPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorPeople'sSpeechPropertyCounts_Top}{RGB}{236,243,242}
\definecolor{color1111HoursHindiPropertyCounts_Top}{RGB}{245,240,226}
\definecolor{colorShrutilipiPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorWenetSpeechPropertyCounts_Top}{RGB}{245,244,244}
\definecolor{colorSamromurChildrenPropertyCounts_Top}{RGB}{245,240,226}
\definecolor{colorSDS-200PropertyCounts_Top}{RGB}{245,233,200}
\definecolor{coloraidatatangPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorFleursPropertyCounts_Top}{RGB}{244,244,244}
\definecolor{colorOLKAVSPropertyCounts_Top}{RGB}{236,243,242}
\definecolor{colorNorwegianParl.PropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorMagicData-RAMCPropertyCounts_Top}{RGB}{235,242,241}
\definecolor{colorKathbathPropertyCounts_Top}{RGB}{245,236,212}
\definecolor{colorHebrewKanPropertyCounts_Top}{RGB}{245,236,212}
\definecolor{colorHebrewCourseraPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorBloomSpeechPropertyCounts_Top}{RGB}{245,243,238}
\definecolor{colorEnglish-VietnamesePropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorEarnings-22PropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorYODASPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorAFRISPEECH-200PropertyCounts_Top}{RGB}{245,241,230}
\definecolor{colorAaltoFinnishParl.PropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorReazonSpeechPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorEdAccPropertyCounts_Top}{RGB}{245,243,238}
\definecolor{colorRixVoxPropertyCounts_Top}{RGB}{245,233,200}
\definecolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{RGB}{245,242,234}
\definecolor{colorSnowMountainPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorSamromurMilljonPropertyCounts_Top}{RGB}{245,240,226}
\definecolor{colorBud500PropertyCounts_Top}{RGB}{245,238,220}
\definecolor{colorVibraVoxPropertyCounts_Top}{RGB}{240,223,178}
\definecolor{colorM2ASRPropertyCounts_Top}{RGB}{245,244,242}

\begin{longtable}{lc|ccccccc|ccc|c}
\caption[\textbf{Audio collections and properties}]{\textbf{Audio collections and properties}. Collection properties include numbers of audio hours (\textsc{HR}), speakers (\textsc{SPKR}), languages (\textsc{Lang}), creator institutions (\textsc{Creat}), tasks (\textsc{Tasks}), data sources (\textsc{Src}), and topics (\textsc{Topics}). The number of datasets is not listed because all collections include only one dataset, except for M2ASR which has four. The \textsc{US} column indicates datasets from or partly from the United States, the \textsc{Ac} column datasets created by academic institutions, and the \textsc{Ind} column datasets created by industry. Note that a dataset can have all of these, none of them, or any combination of them. The \textsc{Use} column indicates whether a collection includes data freely usable even for commercial purposes (\protect\CommercialDataCircle), data usable only for noncommercial purposes or academic research (\protect\NCDataCircle) and data whose license status is not specified precisely enough to allow us to determine commercial use permissions (\protect\UnspecifiedDataCircle). Note that each collection may have different datasets with one, two, or all three of these statuses. Datasets are sorted chronologically to highlight trends over time.} \label{tab:collections-audio} \\
\toprule
\textsc{Collection} & \textsc{} & \multicolumn{7}{c}{\textsc{Property Counts}} & \multicolumn{3}{c}{\textsc{Category}} & \textsc{Perm} \\
 & \textsc{\thead{Year}} & \textsc{\thead{Hr}} & \textsc{\thead{Spkr}} & \textsc{\thead{Lang}} & \textsc{\thead{Creat}} & \textsc{\thead{Tasks}} & \textsc{\thead{Src}} & \textsc{\thead{Top}} & \textsc{\thead{US}} & \textsc{\thead{Ac}} & \textsc{\thead{Ind}} & \textsc{\thead{Use}} \\
\midrule
\endfirsthead
\caption[]{\textbf{Audio collections and properties}.} \\
\toprule
\textsc{Collection} & \textsc{} & \multicolumn{7}{c}{\textsc{Property Counts}} & \multicolumn{3}{c}{\textsc{Category}} & \textsc{Perm} \\
 & \textsc{\thead{Year}} & \textsc{\thead{Hr}} & \textsc{\thead{Spkr}} & \textsc{\thead{Lang}} & \textsc{\thead{Creat}} & \textsc{\thead{Tasks}} & \textsc{\thead{Src}} & \textsc{\thead{Top}} & \textsc{\thead{US}} & \textsc{\thead{Ac}} & \textsc{\thead{Ind}} & \textsc{\thead{Use}} \\
\midrule
\endhead
\midrule
\multicolumn{13}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
TIMIT & 1990 & \cellcolor{colorTIMITPropertyCounts_Hr}{5} & \cellcolor{colorTIMITPropertyCounts_Spkr}{630} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \greencheck & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
Switchboard & 1992 & \cellcolor{colorSwitchboardPropertyCounts_Hr}{250} & \cellcolor{colorSwitchboardPropertyCounts_Spkr}{543} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorSwitchboardPropertyCounts_Top}{70} & \greencheck & \emojiblank & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
African Acc. French & 2003 & \cellcolor{colorAfricanAcc.FrenchPropertyCounts_Hr}{22} & \cellcolor{colorAfricanAcc.FrenchPropertyCounts_Spkr}{232} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
CSJ & 2003 & \cellcolor{colorCSJPropertyCounts_Hr}{661} & \cellcolor{colorCSJPropertyCounts_Spkr}{1k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \emojiblank & \emojiblank & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Fisher & 2004 & \cellcolor{colorFisherPropertyCounts_Hr}{2k} & \cellcolor{colorFisherPropertyCounts_Spkr}{12k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorFisherPropertyCounts_Top}{36} & \greencheck & \greencheck & \emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle \\
CSLU 22 Langs. & 2005 & \cellcolor{colorCSLU22Langs.PropertyCounts_Hr}{84} & - & \cellcolor{colorCSLU22Langs.PropertyCounts_Lang}{21} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \greencheck & \emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle \\
AMI & 2005 & \cellcolor{colorAMIPropertyCounts_Hr}{100} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
CSLU 1.2 & 2007 & \cellcolor{colorMinds14PropertyCounts_Hr}{25} & \cellcolor{colorCSLU1.2PropertyCounts_Spkr}{5k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \greencheck & \emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle \\
ALLSSTAR & 2010 & \cellcolor{colorALLSSTARPropertyCounts_Hr}{86} & \cellcolor{colorALLSSTARPropertyCounts_Spkr}{140} & \cellcolor{colorALLSSTARPropertyCounts_Lang}{27} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorHebrewKanPropertyCounts_Top}{3} & \greencheck & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
TED-LIUM3 & 2012 & \cellcolor{colorTED-LIUM3PropertyCounts_Hr}{452} & \cellcolor{colorTED-LIUM3PropertyCounts_Spkr}{2k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
NST Norwegian & 2013 & \cellcolor{colorNSTNorwegianPropertyCounts_Hr}{540} & \cellcolor{colorNSTNorwegianPropertyCounts_Spkr}{870} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
NST Danish & 2013 & \cellcolor{colorBud500PropertyCounts_Hr}{500} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
NST Swedish & 2013 & \cellcolor{colorNSTSwedishPropertyCounts_Hr}{300} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Vystadial & 2014 & \cellcolor{colorClarinPLPropertyCounts_Hr}{56} & - & \cellcolor{colorEnglish-VietnamesePropertyCounts_Lang}{2} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorHebrewKanPropertyCounts_Top}{3} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
THCHS-30 & 2015 & \cellcolor{colorTHCHS-30PropertyCounts_Hr}{35} & \cellcolor{colorTHCHS-30PropertyCounts_Spkr}{40} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
LibriSpeech & 2015 & \cellcolor{colorM-AILABSPropertyCounts_Hr}{1k} & \cellcolor{colorLibriSpeechPropertyCounts_Spkr}{2k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorLibriSpeechPropertyCounts_Top}{106} & \greencheck & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
THUYG-20 & 2015 & \cellcolor{colorTHUYG-20PropertyCounts_Hr}{20} & \cellcolor{colorTHUYG-20PropertyCounts_Spkr}{371} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorHebrewKanPropertyCounts_Top}{3} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
VCTK & 2016 & \cellcolor{colorVCTKPropertyCounts_Hr}{44} & \cellcolor{colorVCTKPropertyCounts_Spkr}{110} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Spoken Wikipedia & 2016 & \cellcolor{colorSpokenWikipediaPropertyCounts_Hr}{1k} & \cellcolor{colorSpokenWikipediaPropertyCounts_Spkr}{960} & \cellcolor{colorWestAfr.Virt.Asst.PropertyCounts_Lang}{3} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
AISHELL-1 & 2017 & \cellcolor{colorAISHELL-1PropertyCounts_Hr}{520} & \cellcolor{colorAISHELL-1PropertyCounts_Spkr}{400} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorFleursPropertyCounts_Top}{11} & \emojiblank & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
LJSpeech & 2017 & \cellcolor{colorLJSpeechPropertyCounts_Hr}{24} & \cellcolor{colorLJSpeechPropertyCounts_Spkr}{1} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
ClarinPL & 2017 & \cellcolor{colorClarinPLPropertyCounts_Hr}{56} & \cellcolor{colorClarinPLPropertyCounts_Spkr}{317} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
AISHELL-2 & 2018 & \cellcolor{colorM-AILABSPropertyCounts_Hr}{1k} & \cellcolor{colorAISHELL-2PropertyCounts_Spkr}{2k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorEdAccPropertyCounts_Top}{8} & \emojiblank & \emojiblank & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Regional Af. Am. Lang. & 2018 & \cellcolor{colorRegionalAf.Am.Lang.PropertyCounts_Hr}{159} & \cellcolor{colorRegionalAf.Am.Lang.PropertyCounts_Spkr}{222} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorEdAccPropertyCounts_Top}{8} & \greencheck & \greencheck & \emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle \\
Crowd Sourced Speech & 2018 & \cellcolor{colorCrowdSourcedSpeechPropertyCounts_Hr}{1k} & \cellcolor{colorCrowdSourcedSpeechPropertyCounts_Spkr}{3k} & \cellcolor{colorCrowdSourcedSpeechPropertyCounts_Lang}{5} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Zeroth-Korean & 2018 & \cellcolor{colorZeroth-KoreanPropertyCounts_Hr}{96} & \cellcolor{colorZeroth-KoreanPropertyCounts_Spkr}{181} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
RTVE & 2018 & \cellcolor{colorRTVEPropertyCounts_Hr}{691} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \greencheck & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
OpenSTT & 2019 & \cellcolor{colorOpenSTTPropertyCounts_Hr}{20k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Top}{6} & \emojiblank & \greencheck & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
MuST-C & 2019 & \cellcolor{colorMuST-CPropertyCounts_Hr}{4k} & \cellcolor{colorMuST-CPropertyCounts_Spkr}{2k} & \cellcolor{colorVoxPopuliPropertyCounts_Lang}{16} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorBud500PropertyCounts_Top}{4} & \emojiblank & \greencheck & \emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle \\
M-AILABS & 2019 & \cellcolor{colorM-AILABSPropertyCounts_Hr}{1k} & - & \cellcolor{colorMaSSPropertyCounts_Lang}{8} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorMultiling.LibriSpeechPropertyCounts_Top}{33} & \emojiblank & \emojiblank & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
MAGICDATA & 2019 & \cellcolor{colorMAGICDATAPropertyCounts_Hr}{755} & \cellcolor{colorMAGICDATAPropertyCounts_Spkr}{1k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \emojiblank & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
Common Voice 17 & 2019 & \cellcolor{colorCommonVoice17PropertyCounts_Hr}{31k} & \cellcolor{colorCommonVoice17PropertyCounts_Spkr}{330k} & \cellcolor{colorCommonVoice17PropertyCounts_Lang}{124} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
CoNASE & 2019 & \cellcolor{colorCoNASEPropertyCounts_Hr}{154k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Top}{6} & \emojiblank & \greencheck & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Nigerian English & 2019 & \cellcolor{colorNigerianEnglishPropertyCounts_Hr}{6} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Norwegian Parl. Speech & 2019 & \cellcolor{colorNorwegianParl.PropertyCounts_Hr}{140} & \cellcolor{colorNorwegianParl.SpeechPropertyCounts_Spkr}{309} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
120h Spanish Speech & 2019 & \cellcolor{colorAISHELL-4PropertyCounts_Hr}{120} & \cellcolor{color120hSpanishSpeechPropertyCounts_Spkr}{17} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
DiDiSpeech & 2020 & \cellcolor{colorDiDiSpeechPropertyCounts_Hr}{800} & \cellcolor{colorDiDiSpeechPropertyCounts_Spkr}{6k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \emojiblank & \emojiblank & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Czech Parliament & 2020 & \cellcolor{colorCzechParliamentPropertyCounts_Hr}{444} & \cellcolor{colorCzechParliamentPropertyCounts_Spkr}{212} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
CoVoST-2 & 2020 & \cellcolor{colorCoVoST-2PropertyCounts_Hr}{3k} & \cellcolor{colorCoVoST-2PropertyCounts_Spkr}{78k} & \cellcolor{colorCoVoST-2PropertyCounts_Lang}{22} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
KSC & 2020 & \cellcolor{colorKSCPropertyCounts_Hr}{332} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorSamromurMilljonPropertyCounts_Top}{5} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Basq., Cat. and Gal. & 2020 & \cellcolor{colorBasq.,Cat.andGal.PropertyCounts_Hr}{34} & \cellcolor{colorBasq.,Cat.andGal.PropertyCounts_Spkr}{132} & \cellcolor{colorWestAfr.Virt.Asst.PropertyCounts_Lang}{3} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \greencheck & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
KsponSpeech & 2020 & \cellcolor{colorKsponSpeechPropertyCounts_Hr}{969} & \cellcolor{colorKsponSpeechPropertyCounts_Spkr}{2k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Top}{6} & \emojiblank & \emojiblank & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Samromur & 2020 & \cellcolor{colorSamromurPropertyCounts_Hr}{145} & \cellcolor{colorSamromurPropertyCounts_Spkr}{8k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorSamromurMilljonPropertyCounts_Top}{5} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Multiling. LibriSpeech & 2020 & \cellcolor{colorMultiling.LibriSpeechPropertyCounts_Hr}{50k} & \cellcolor{colorMultiling.LibriSpeechPropertyCounts_Spkr}{6k} & \cellcolor{colorMaSSPropertyCounts_Lang}{8} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorMultiling.LibriSpeechPropertyCounts_Top}{33} & \greencheck & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
MaSS & 2020 & \cellcolor{colorMaSSPropertyCounts_Hr}{160} & - & \cellcolor{colorMaSSPropertyCounts_Lang}{8} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
FT SPEECH & 2020 & \cellcolor{colorFTSPEECHPropertyCounts_Hr}{2k} & \cellcolor{colorFTSPEECHPropertyCounts_Spkr}{434} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \greencheck & \greencheck & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Eng. Acc. in Brit. Isles & 2020 & \cellcolor{colorEng.Acc.inBrit.IslesPropertyCounts_Hr}{31} & \cellcolor{colorEdAccPropertyCounts_Spkr}{120} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorBud500PropertyCounts_Top}{4} & \emojiblank & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Highland Puebla Nahuatl & 2021 & \cellcolor{colorHighlandPueblaNahuatlPropertyCounts_Hr}{156} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \greencheck & \emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle \\
QASR & 2021 & \cellcolor{colorQASRPropertyCounts_Hr}{2k} & \cellcolor{colorQASRPropertyCounts_Spkr}{11k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \greencheck & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Multiling. TEDx & 2021 & \cellcolor{colorMultiling.TEDxPropertyCounts_Hr}{765} & - & \cellcolor{colorMultiling.TEDxPropertyCounts_Lang}{9} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \greencheck & \emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle \\
Minds14 & 2021 & \cellcolor{colorMinds14PropertyCounts_Hr}{25} & - & \cellcolor{colorSnowMountainPropertyCounts_Lang}{14} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Golos & 2021 & \cellcolor{colorGolosPropertyCounts_Hr}{1k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Top}{6} & \emojiblank & \greencheck & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
MASC & 2021 & \cellcolor{colorMASCPropertyCounts_Hr}{1k} & \cellcolor{colorMASCPropertyCounts_Spkr}{14k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorMagicData-RAMCPropertyCounts_Top}{15} & \emojiblank & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
LaboroTVSpeech & 2021 & \cellcolor{colorLaboroTVSpeechPropertyCounts_Hr}{2k} & - & \cellcolor{colorEnglish-VietnamesePropertyCounts_Lang}{2} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \greencheck & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
KeSpeech & 2021 & \cellcolor{colorKeSpeechPropertyCounts_Hr}{2k} & \cellcolor{colorKeSpeechPropertyCounts_Spkr}{27k} & \cellcolor{colorEnglish-VietnamesePropertyCounts_Lang}{2} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
JTUBESPEECH & 2021 & \cellcolor{colorJTUBESPEECHPropertyCounts_Hr}{1k} & - & \cellcolor{colorEnglish-VietnamesePropertyCounts_Lang}{2} & \cellcolor{colorMagicData-RAMCPropertyCounts_Creat}{4} & \cellcolor{colorMagicData-RAMCPropertyCounts_Tasks}{4} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \greencheck & \greencheck & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
GigaSpeech & 2021 & \cellcolor{colorGigaSpeechPropertyCounts_Hr}{10k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorGigaSpeechPropertyCounts_Creat}{9} & \cellcolor{colorGigaSpeechPropertyCounts_Tasks}{9} & \cellcolor{colorEarnings-22PropertyCounts_Src}{3} & \cellcolor{colorGigaSpeechPropertyCounts_Top}{24} & \greencheck & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
VoxPopuli & 2021 & \cellcolor{colorVoxPopuliPropertyCounts_Hr}{2k} & \cellcolor{colorVoxPopuliPropertyCounts_Spkr}{4k} & \cellcolor{colorVoxPopuliPropertyCounts_Lang}{16} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
SPGISpeech & 2021 & \cellcolor{colorSPGISpeechPropertyCounts_Hr}{5k} & \cellcolor{colorSPGISpeechPropertyCounts_Spkr}{50k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorMagicData-RAMCPropertyCounts_Creat}{4} & \cellcolor{colorMagicData-RAMCPropertyCounts_Tasks}{4} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \greencheck & \greencheck & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
West Afr. Radio & 2021 & \cellcolor{colorWestAfr.RadioPropertyCounts_Hr}{142} & - & \cellcolor{colorWestAfr.RadioPropertyCounts_Lang}{10} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorHebrewKanPropertyCounts_Top}{3} & \greencheck & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
AISHELL-4 & 2021 & \cellcolor{colorAISHELL-4PropertyCounts_Hr}{120} & \cellcolor{colorAISHELL-4PropertyCounts_Spkr}{61} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorMagicData-RAMCPropertyCounts_Creat}{4} & \cellcolor{colorMagicData-RAMCPropertyCounts_Tasks}{4} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Top}{6} & \greencheck & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
West Afr. Virt. Asst. & 2021 & \cellcolor{colorWestAfr.Virt.Asst.PropertyCounts_Hr}{2} & \cellcolor{colorWestAfr.Virt.Asst.PropertyCounts_Spkr}{49} & \cellcolor{colorWestAfr.Virt.Asst.PropertyCounts_Lang}{3} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \greencheck & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
MediaSpeech & 2021 & \cellcolor{colorEdAccPropertyCounts_Hr}{40} & - & \cellcolor{colorM2ASRPropertyCounts_Lang}{4} & \cellcolor{colorBloomSpeechPropertyCounts_Creat}{5} & \cellcolor{colorBloomSpeechPropertyCounts_Tasks}{5} & \cellcolor{colorMediaSpeechPropertyCounts_Src}{12} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
People's Speech & 2021 & \cellcolor{colorPeople'sSpeechPropertyCounts_Hr}{30k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorPeople'sSpeechPropertyCounts_Creat}{7} & \cellcolor{colorPeople'sSpeechPropertyCounts_Tasks}{7} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorOLKAVSPropertyCounts_Top}{14} & \greencheck & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
1111 Hours Hindi & 2022 & \cellcolor{color1111HoursHindiPropertyCounts_Hr}{108} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorSamromurMilljonPropertyCounts_Top}{5} & \emojiblank & \emojiblank & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Shrutilipi & 2022 & \cellcolor{colorShrutilipiPropertyCounts_Hr}{6k} & - & \cellcolor{colorKathbathPropertyCounts_Lang}{12} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
WenetSpeech & 2022 & \cellcolor{colorWenetSpeechPropertyCounts_Hr}{10k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorMagicData-RAMCPropertyCounts_Creat}{4} & \cellcolor{colorMagicData-RAMCPropertyCounts_Tasks}{4} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorWenetSpeechPropertyCounts_Top}{10} & \emojiblank & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Samromur Children & 2022 & \cellcolor{colorSamromurChildrenPropertyCounts_Hr}{131} & \cellcolor{colorSamromurChildrenPropertyCounts_Spkr}{3k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorSamromurMilljonPropertyCounts_Top}{5} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
SDS-200 & 2022 & \cellcolor{colorAFRISPEECH-200PropertyCounts_Hr}{200} & \cellcolor{colorSDS-200PropertyCounts_Spkr}{4k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \emojiblank & \greencheck & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
aidatatang & 2022 & \cellcolor{colorAFRISPEECH-200PropertyCounts_Hr}{200} & \cellcolor{coloraidatatangPropertyCounts_Spkr}{600} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
Fleurs & 2022 & \cellcolor{colorFleursPropertyCounts_Hr}{1k} & - & \cellcolor{colorFleursPropertyCounts_Lang}{102} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorFleursPropertyCounts_Top}{11} & \greencheck & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
OLKAVS & 2022 & \cellcolor{colorOLKAVSPropertyCounts_Hr}{1k} & \cellcolor{colorOLKAVSPropertyCounts_Spkr}{1k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorOLKAVSPropertyCounts_Top}{14} & \emojiblank & \greencheck & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Norwegian Parl. & 2022 & \cellcolor{colorNorwegianParl.PropertyCounts_Hr}{140} & \cellcolor{colorNorwegianParl.PropertyCounts_Spkr}{267} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \emojiblank & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
MagicData-RAMC & 2022 & \cellcolor{colorMagicData-RAMCPropertyCounts_Hr}{180} & \cellcolor{colorMagicData-RAMCPropertyCounts_Spkr}{663} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorMagicData-RAMCPropertyCounts_Creat}{4} & \cellcolor{colorMagicData-RAMCPropertyCounts_Tasks}{4} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorMagicData-RAMCPropertyCounts_Top}{15} & \emojiblank & \greencheck & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
Kathbath & 2022 & \cellcolor{colorKathbathPropertyCounts_Hr}{2k} & \cellcolor{colorKathbathPropertyCounts_Spkr}{1k} & \cellcolor{colorKathbathPropertyCounts_Lang}{12} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorHebrewKanPropertyCounts_Top}{3} & \emojiblank & \greencheck & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Hebrew Kan & 2022 & \cellcolor{colorHebrewKanPropertyCounts_Hr}{9} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorHebrewKanPropertyCounts_Top}{3} & \emojiblank & \emojiblank & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Hebrew Coursera & 2022 & \cellcolor{colorHebrewCourseraPropertyCounts_Hr}{36} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
Bloom Speech & 2022 & \cellcolor{colorBloomSpeechPropertyCounts_Hr}{428} & - & \cellcolor{colorBloomSpeechPropertyCounts_Lang}{56} & \cellcolor{colorBloomSpeechPropertyCounts_Creat}{5} & \cellcolor{colorBloomSpeechPropertyCounts_Tasks}{5} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorEdAccPropertyCounts_Top}{8} & \greencheck & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \NCDataCircle \\
English-Vietnamese & 2022 & \cellcolor{colorEnglish-VietnamesePropertyCounts_Hr}{508} & - & \cellcolor{colorEnglish-VietnamesePropertyCounts_Lang}{2} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
Earnings-22 & 2022 & \cellcolor{colorEarnings-22PropertyCounts_Hr}{119} & \cellcolor{colorEarnings-22PropertyCounts_Spkr}{125} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorEarnings-22PropertyCounts_Src}{3} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \greencheck & \emojiblank & \greencheck & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
YODAS & 2023 & \cellcolor{colorYODASPropertyCounts_Hr}{370k} & - & \cellcolor{colorYODASPropertyCounts_Lang}{149} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
AFRISPEECH-200 & 2023 & \cellcolor{colorAFRISPEECH-200PropertyCounts_Hr}{200} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Spkr}{2k} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Lang}{20} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Creat}{14} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Tasks}{14} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorAFRISPEECH-200PropertyCounts_Top}{6} & \greencheck & \greencheck & \greencheck & \TransparentCircle \TransparentCircle \NCDataCircle \\
Aalto Finnish Parl. & 2023 & \cellcolor{colorAaltoFinnishParl.PropertyCounts_Hr}{3k} & \cellcolor{colorAaltoFinnishParl.PropertyCounts_Spkr}{449} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \emojiblank & \greencheck & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
ReazonSpeech & 2023 & \cellcolor{colorReazonSpeechPropertyCounts_Hr}{35k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
EdAcc & 2023 & \cellcolor{colorEdAccPropertyCounts_Hr}{40} & \cellcolor{colorEdAccPropertyCounts_Spkr}{120} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorEdAccPropertyCounts_Top}{8} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
RixVox & 2023 & \cellcolor{colorRixVoxPropertyCounts_Hr}{5k} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorRixVoxPropertyCounts_Top}{2} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Japanese Anime Speech & 2023 & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Hr}{110} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorJapaneseAnimeSpeechPropertyCounts_Top}{7} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Snow Mountain & 2023 & \cellcolor{colorSnowMountainPropertyCounts_Hr}{273} & \cellcolor{colorSnowMountainPropertyCounts_Spkr}{11} & \cellcolor{colorSnowMountainPropertyCounts_Lang}{14} & \cellcolor{colorSnowMountainPropertyCounts_Creat}{2} & \cellcolor{colorSnowMountainPropertyCounts_Tasks}{2} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \greencheck & \emojiblank & \greencheck & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Samromur Milljon & 2023 & \cellcolor{colorSamromurMilljonPropertyCounts_Hr}{967} & \cellcolor{colorSamromurMilljonPropertyCounts_Spkr}{17k} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorSamromurMilljonPropertyCounts_Top}{5} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
Bud500 & 2024 & \cellcolor{colorBud500PropertyCounts_Hr}{500} & - & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorBud500PropertyCounts_Src}{2} & \cellcolor{colorBud500PropertyCounts_Top}{4} & \emojiblank & \emojiblank & \emojiblank & \CommercialDataCircle \TransparentCircle \NCDataCircle \\
VibraVox & 2024 & \cellcolor{colorVibraVoxPropertyCounts_Hr}{18} & \cellcolor{colorVibraVoxPropertyCounts_Spkr}{200} & \cellcolor{colorVibraVoxPropertyCounts_Lang}{1} & \cellcolor{colorVibraVoxPropertyCounts_Creat}{1} & \cellcolor{colorVibraVoxPropertyCounts_Tasks}{1} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorVibraVoxPropertyCounts_Top}{1} & \emojiblank & \greencheck & \emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle \\
M2ASR & Mult. & \cellcolor{colorM2ASRPropertyCounts_Hr}{448} & \cellcolor{colorM2ASRPropertyCounts_Spkr}{655} & \cellcolor{colorM2ASRPropertyCounts_Lang}{4} & \cellcolor{colorM2ASRPropertyCounts_Creat}{3} & \cellcolor{colorM2ASRPropertyCounts_Tasks}{3} & \cellcolor{colorM2ASRPropertyCounts_Src}{1} & \cellcolor{colorM2ASRPropertyCounts_Top}{9} & \emojiblank & \greencheck & \emojiblank & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle \\
\end{longtable}


==> tables/collections-text.tex <==
\setlength{\tabcolsep}{1.9pt}
\definecolor{colorRiddleSensePropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorFeedbackColl.PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorNectarPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMetaMathQAPropertyCounts_Datasets}{RGB}{245,244,242}
\definecolor{colorMegaWikaPropertyCounts_Datasets}{RGB}{200,234,229}
\definecolor{colorOpenGPTHealthcarePropertyCounts_Datasets}{RGB}{245,236,212}
\definecolor{colorMedInstr.PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMathInstr.PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMathDialPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorUltraFeedbackArgillaPropertyCounts_Datasets}{RGB}{245,244,244}
\definecolor{colorLMSYS-Chat-1MPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorPII-Masking-200kPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHelpSteerPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorPure-DovePropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorGlaiveCodeAsst.PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorNoRobotsPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorOpenAsst.v2PropertyCounts_Datasets}{RGB}{226,240,238}
\definecolor{colorEverythingLMPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorUltraChat-200kPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorThaiGenAIPropertyCounts_Datasets}{RGB}{245,244,244}
\definecolor{colorBactrian-XPropertyCounts_Datasets}{RGB}{245,241,232}
\definecolor{colorCOBRAFramesPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorSelFeePropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCapybaraPropertyCounts_Datasets}{RGB}{240,243,243}
\definecolor{colorExpertQAPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorChatDoctorPropertyCounts_Datasets}{RGB}{245,236,212}
\definecolor{colorSeaBenchPropertyCounts_Datasets}{RGB}{245,244,244}
\definecolor{colorCollectiveCognitionPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorDeita10KPropertyCounts_Datasets}{RGB}{245,234,202}
\definecolor{colorPygmalionAI-PIPPAPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorChatbotArenaPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorOpenMathInstr.-1PropertyCounts_Datasets}{RGB}{245,234,202}
\definecolor{colorOrca-MathPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{color10kPromptRankedPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorLongAlign-10kPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorLlama2-MedTuned-Instr.PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorKIWIPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorIndic-Instr.PropertyCounts_Datasets}{RGB}{245,244,242}
\definecolor{colorGretelText-to-SQLPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorConiferPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCidarPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorAyaPropertyCounts_Datasets}{RGB}{187,229,223}
\definecolor{colorWildChatPropertyCounts_Datasets}{RGB}{245,234,202}
\definecolor{colorMedicalMeadowPropertyCounts_Datasets}{RGB}{245,244,242}
\definecolor{colorPMC-LLaMAInstr.PropertyCounts_Datasets}{RGB}{245,243,238}
\definecolor{colorDialogStudioPropertyCounts_Datasets}{RGB}{179,226,219}
\definecolor{colorCOIGPropertyCounts_Datasets}{RGB}{227,240,239}
\definecolor{colorAgentInstructPropertyCounts_Datasets}{RGB}{245,241,232}
\definecolor{colorOpen-PlatypusPropertyCounts_Datasets}{RGB}{242,244,244}
\definecolor{colorRiddleSensePropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorFeedbackColl.PropertyCounts_Tasks}{RGB}{245,236,212}
\definecolor{colorNectarPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorMetaMathQAPropertyCounts_Tasks}{RGB}{245,236,212}
\definecolor{colorMegaWikaPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorOpenGPTHealthcarePropertyCounts_Tasks}{RGB}{245,244,244}
\definecolor{colorMedInstr.PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorMathInstr.PropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorMathDialPropertyCounts_Tasks}{RGB}{245,236,212}
\definecolor{colorUltraFeedbackArgillaPropertyCounts_Tasks}{RGB}{185,228,221}
\definecolor{colorLMSYS-Chat-1MPropertyCounts_Tasks}{RGB}{213,237,234}
\definecolor{colorPII-Masking-200kPropertyCounts_Tasks}{RGB}{245,236,212}
\definecolor{colorHelpSteerPropertyCounts_Tasks}{RGB}{236,243,242}
\definecolor{colorPure-DovePropertyCounts_Tasks}{RGB}{245,244,244}
\definecolor{colorGlaiveCodeAsst.PropertyCounts_Tasks}{RGB}{245,236,212}
\definecolor{colorNoRobotsPropertyCounts_Tasks}{RGB}{218,238,235}
\definecolor{colorOpenAsst.v2PropertyCounts_Tasks}{RGB}{245,244,244}
\definecolor{colorEverythingLMPropertyCounts_Tasks}{RGB}{218,238,235}
\definecolor{colorUltraChat-200kPropertyCounts_Tasks}{RGB}{224,240,237}
\definecolor{colorThaiGenAIPropertyCounts_Tasks}{RGB}{204,235,230}
\definecolor{colorBactrian-XPropertyCounts_Tasks}{RGB}{245,244,244}
\definecolor{colorCOBRAFramesPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorSelFeePropertyCounts_Tasks}{RGB}{236,243,242}
\definecolor{colorCapybaraPropertyCounts_Tasks}{RGB}{179,226,219}
\definecolor{colorExpertQAPropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorChatDoctorPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorSeaBenchPropertyCounts_Tasks}{RGB}{245,244,244}
\definecolor{colorCollectiveCognitionPropertyCounts_Tasks}{RGB}{229,241,239}
\definecolor{colorDeita10KPropertyCounts_Tasks}{RGB}{204,235,230}
\definecolor{colorPygmalionAI-PIPPAPropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorChatbotArenaPropertyCounts_Tasks}{RGB}{245,244,244}
\definecolor{colorOpenMathInstr.-1PropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorOrca-MathPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{color10kPromptRankedPropertyCounts_Tasks}{RGB}{199,234,229}
\definecolor{colorLongAlign-10kPropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{RGB}{245,244,244}
\definecolor{colorKIWIPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorIndic-Instr.PropertyCounts_Tasks}{RGB}{224,240,237}
\definecolor{colorGretelText-to-SQLPropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorConiferPropertyCounts_Tasks}{RGB}{218,238,235}
\definecolor{colorCidarPropertyCounts_Tasks}{RGB}{218,238,235}
\definecolor{colorAyaPropertyCounts_Tasks}{RGB}{224,240,237}
\definecolor{colorWildChatPropertyCounts_Tasks}{RGB}{224,240,237}
\definecolor{colorMedicalMeadowPropertyCounts_Tasks}{RGB}{245,236,212}
\definecolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{RGB}{240,223,178}
\definecolor{colorDialogStudioPropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorCOIGPropertyCounts_Tasks}{RGB}{199,234,229}
\definecolor{colorAgentInstructPropertyCounts_Tasks}{RGB}{245,241,230}
\definecolor{colorOpen-PlatypusPropertyCounts_Tasks}{RGB}{208,236,232}
\definecolor{colorRiddleSensePropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorFeedbackColl.PropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorNectarPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorMetaMathQAPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorMegaWikaPropertyCounts_Langs}{RGB}{196,232,227}
\definecolor{colorOpenGPTHealthcarePropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorMedInstr.PropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorMathInstr.PropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorMathDialPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorUltraFeedbackArgillaPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorLMSYS-Chat-1MPropertyCounts_Langs}{RGB}{245,241,230}
\definecolor{colorPII-Masking-200kPropertyCounts_Langs}{RGB}{245,239,222}
\definecolor{colorHelpSteerPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorPure-DovePropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorGlaiveCodeAsst.PropertyCounts_Langs}{RGB}{245,234,202}
\definecolor{colorNoRobotsPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorOpenAsst.v2PropertyCounts_Langs}{RGB}{222,239,237}
\definecolor{colorEverythingLMPropertyCounts_Langs}{RGB}{245,234,202}
\definecolor{colorUltraChat-200kPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorThaiGenAIPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorBactrian-XPropertyCounts_Langs}{RGB}{245,242,234}
\definecolor{colorCOBRAFramesPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorSelFeePropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorCapybaraPropertyCounts_Langs}{RGB}{245,234,202}
\definecolor{colorExpertQAPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorChatDoctorPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorSeaBenchPropertyCounts_Langs}{RGB}{244,244,244}
\definecolor{colorCollectiveCognitionPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorDeita10KPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorPygmalionAI-PIPPAPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorChatbotArenaPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorOpenMathInstr.-1PropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorOrca-MathPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{color10kPromptRankedPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorLongAlign-10kPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorLlama2-MedTuned-Instr.PropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorKIWIPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorIndic-Instr.PropertyCounts_Langs}{RGB}{245,234,202}
\definecolor{colorGretelText-to-SQLPropertyCounts_Langs}{RGB}{245,237,214}
\definecolor{colorConiferPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorCidarPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorAyaPropertyCounts_Langs}{RGB}{179,226,219}
\definecolor{colorWildChatPropertyCounts_Langs}{RGB}{240,243,243}
\definecolor{colorMedicalMeadowPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorPMC-LLaMAInstr.PropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorDialogStudioPropertyCounts_Langs}{RGB}{245,241,230}
\definecolor{colorCOIGPropertyCounts_Langs}{RGB}{245,234,202}
\definecolor{colorAgentInstructPropertyCounts_Langs}{RGB}{240,223,178}
\definecolor{colorOpen-PlatypusPropertyCounts_Langs}{RGB}{206,235,231}
\definecolor{colorRiddleSensePropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorFeedbackColl.PropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorNectarPropertyCounts_Domains}{RGB}{245,236,210}
\definecolor{colorMetaMathQAPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorMegaWikaPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorOpenGPTHealthcarePropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorMedInstr.PropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorMathInstr.PropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorMathDialPropertyCounts_Domains}{RGB}{245,243,238}
\definecolor{colorUltraFeedbackArgillaPropertyCounts_Domains}{RGB}{185,228,221}
\definecolor{colorLMSYS-Chat-1MPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorPII-Masking-200kPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorHelpSteerPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorPure-DovePropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorGlaiveCodeAsst.PropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorNoRobotsPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorOpenAsst.v2PropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorEverythingLMPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorUltraChat-200kPropertyCounts_Domains}{RGB}{245,236,210}
\definecolor{colorThaiGenAIPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorBactrian-XPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorCOBRAFramesPropertyCounts_Domains}{RGB}{245,236,210}
\definecolor{colorSelFeePropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorCapybaraPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorExpertQAPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorChatDoctorPropertyCounts_Domains}{RGB}{245,236,210}
\definecolor{colorSeaBenchPropertyCounts_Domains}{RGB}{242,244,244}
\definecolor{colorCollectiveCognitionPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorDeita10KPropertyCounts_Domains}{RGB}{245,240,226}
\definecolor{colorPygmalionAI-PIPPAPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorChatbotArenaPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorOpenMathInstr.-1PropertyCounts_Domains}{RGB}{245,240,226}
\definecolor{colorOrca-MathPropertyCounts_Domains}{RGB}{245,240,226}
\definecolor{color10kPromptRankedPropertyCounts_Domains}{RGB}{245,243,238}
\definecolor{colorLongAlign-10kPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorLlama2-MedTuned-Instr.PropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorKIWIPropertyCounts_Domains}{RGB}{245,236,210}
\definecolor{colorIndic-Instr.PropertyCounts_Domains}{RGB}{245,240,226}
\definecolor{colorGretelText-to-SQLPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorConiferPropertyCounts_Domains}{RGB}{245,236,210}
\definecolor{colorCidarPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorAyaPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorWildChatPropertyCounts_Domains}{RGB}{240,223,178}
\definecolor{colorMedicalMeadowPropertyCounts_Domains}{RGB}{245,240,226}
\definecolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{RGB}{245,236,210}
\definecolor{colorDialogStudioPropertyCounts_Domains}{RGB}{245,240,226}
\definecolor{colorCOIGPropertyCounts_Domains}{RGB}{179,226,219}
\definecolor{colorAgentInstructPropertyCounts_Domains}{RGB}{229,241,239}
\definecolor{colorOpen-PlatypusPropertyCounts_Domains}{RGB}{224,240,237}

\begin{longtable}{lc|cccc|c|cc}
\caption[\textbf{Alignment tuning (text) collections and properties}]{\textbf{Alignment tuning (text) collections and properties}. Collection properties include numbers of datasets, tasks, languages, and text domains. The \textsc{Source} column indicates whether a collection contains human-generated web text (\emoji{globe-with-meridians}), language model outputs (\emoji{robot}) or both (\emoji{globe-with-meridians}\emoji{robot}). The \textsc{Use} column indicates whether a collection includes data freely usable even for commercial purposes (\protect\CommercialDataCircle), data usable only for noncommercial purposes or academic research (\protect\NCDataCircle) and data whose license status is not specified precisely enough to allow us to determine commercial use permissions (\protect\UnspecifiedDataCircle). Note that each collection may have different datasets with one, two, or all three of these statuses. Finally, the \textsc{OAI} column indicates collections which include OpenAI model generations. Datasets are sorted chronologically to highlight trends over time.} \label{tab:collections-text} \\
\toprule
\textsc{Collection} & \textsc{} & \multicolumn{4}{c}{\textsc{Property Counts}} & \textsc{Types} & \multicolumn{2}{c}{\textsc{Permissions}} \\
 & \textsc{\thead{Year}} & \textsc{\thead{Datasets}} & \textsc{\thead{Tasks}} & \textsc{\thead{Langs}} & \textsc{\thead{Domains}} & \textsc{\thead{Source}} & \textsc{\thead{Use}} & \textsc{\thead{OAI}} \\
\midrule
\endfirsthead
\caption[]{\textbf{Alignment tuning (text) collections and properties}.} \\
\toprule
\textsc{Collection} & \textsc{} & \multicolumn{4}{c}{\textsc{Property Counts}} & \textsc{Types} & \multicolumn{2}{c}{\textsc{Permissions}} \\
 & \textsc{\thead{Year}} & \textsc{\thead{Datasets}} & \textsc{\thead{Tasks}} & \textsc{\thead{Langs}} & \textsc{\thead{Domains}} & \textsc{\thead{Source}} & \textsc{\thead{Use}} & \textsc{\thead{OAI}} \\
\midrule
\endhead
\midrule
\multicolumn{9}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
RiddleSense & 2021 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emoji{globe-with-meridians}\emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
Feedback Coll. & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorMedicalMeadowPropertyCounts_Tasks}{2} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Nectar & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{2} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
MetaMathQA & 2023 & \cellcolor{colorMedicalMeadowPropertyCounts_Datasets}{8} & \cellcolor{colorMedicalMeadowPropertyCounts_Tasks}{2} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
MegaWika & 2023 & \cellcolor{colorMegaWikaPropertyCounts_Datasets}{50} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorMegaWikaPropertyCounts_Langs}{50} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
OpenGPT Healthcare & 2023 & \cellcolor{colorChatDoctorPropertyCounts_Datasets}{3} & \cellcolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{4} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
MedInstr. & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
MathInstr. & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
MathDial & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorMedicalMeadowPropertyCounts_Tasks}{2} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{color10kPromptRankedPropertyCounts_Domains}{4} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
UltraFeedback Argilla & 2023 & \cellcolor{colorSeaBenchPropertyCounts_Datasets}{9} & \cellcolor{colorUltraFeedbackArgillaPropertyCounts_Tasks}{16} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorUltraFeedbackArgillaPropertyCounts_Domains}{20} & \emoji{globe-with-meridians}\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \NCDataCircle & \greencheck \\
LMSYS-Chat-1M & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorLMSYS-Chat-1MPropertyCounts_Tasks}{9} & \cellcolor{colorDialogStudioPropertyCounts_Langs}{5} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
PII-Masking-200k & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorMedicalMeadowPropertyCounts_Tasks}{2} & \cellcolor{colorPII-Masking-200kPropertyCounts_Langs}{4} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emoji{globe-with-meridians}\emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle & \emojiblank \\
HelpSteer & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorSelFeePropertyCounts_Tasks}{5} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emoji{globe-with-meridians}\emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
Pure-Dove & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{4} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Glaive Code Asst. & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorMedicalMeadowPropertyCounts_Tasks}{2} & \cellcolor{colorCOIGPropertyCounts_Langs}{2} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
No Robots & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorCidarPropertyCounts_Tasks}{8} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emoji{globe-with-meridians}\emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle & \emojiblank \\
Open Asst. v2 & 2023 & \cellcolor{colorOpenAsst.v2PropertyCounts_Datasets}{19} & \cellcolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{4} & \cellcolor{colorOpenAsst.v2PropertyCounts_Langs}{19} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emoji{globe-with-meridians}\emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
EverythingLM & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorCidarPropertyCounts_Tasks}{8} & \cellcolor{colorCOIGPropertyCounts_Langs}{2} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
UltraChat-200k & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorWildChatPropertyCounts_Tasks}{7} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{2} & \emojiblank\emoji{robot} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
Thai Gen AI & 2023 & \cellcolor{colorSeaBenchPropertyCounts_Datasets}{9} & \cellcolor{colorDeita10KPropertyCounts_Tasks}{11} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
Bactrian-X & 2023 & \cellcolor{colorAgentInstructPropertyCounts_Datasets}{6} & \cellcolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{4} & \cellcolor{colorBactrian-XPropertyCounts_Langs}{6} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
COBRA Frames & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{2} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
SelFee & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorSelFeePropertyCounts_Tasks}{5} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Capybara & 2023 & \cellcolor{colorCapybaraPropertyCounts_Datasets}{11} & \cellcolor{colorCapybaraPropertyCounts_Tasks}{17} & \cellcolor{colorCOIGPropertyCounts_Langs}{2} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \NCDataCircle & \greencheck \\
ExpertQA & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
ChatDoctor & 2023 & \cellcolor{colorChatDoctorPropertyCounts_Datasets}{3} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{2} & \emoji{globe-with-meridians}\emoji{robot} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
SeaBench & 2023 & \cellcolor{colorSeaBenchPropertyCounts_Datasets}{9} & \cellcolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{4} & \cellcolor{colorSeaBenchPropertyCounts_Langs}{9} & \cellcolor{colorSeaBenchPropertyCounts_Domains}{5} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
CollectiveCognition & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorCollectiveCognitionPropertyCounts_Tasks}{6} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Deita 10K & 2023 & \cellcolor{colorWildChatPropertyCounts_Datasets}{2} & \cellcolor{colorDeita10KPropertyCounts_Tasks}{11} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorDialogStudioPropertyCounts_Domains}{3} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
PygmalionAI-PIPPA & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
ChatbotArena & 2023 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{4} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
OpenMathInstr.-1 & 2024 & \cellcolor{colorWildChatPropertyCounts_Datasets}{2} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorDialogStudioPropertyCounts_Domains}{3} & \emojiblank\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \TransparentCircle & \emojiblank \\
Orca-Math & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorDialogStudioPropertyCounts_Domains}{3} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
10k Prompt Ranked & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorCOIGPropertyCounts_Tasks}{13} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{color10kPromptRankedPropertyCounts_Domains}{4} & \emojiblank\emoji{robot} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
LongAlign-10k & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \NCDataCircle & \greencheck \\
Llama2-MedTuned-Instr. & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorLlama2-MedTuned-Instr.PropertyCounts_Tasks}{4} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emoji{globe-with-meridians}\emojiblank & \TransparentCircle \TransparentCircle \NCDataCircle & \emojiblank \\
KIWI & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{2} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Indic-Instr. & 2024 & \cellcolor{colorMedicalMeadowPropertyCounts_Datasets}{8} & \cellcolor{colorWildChatPropertyCounts_Tasks}{7} & \cellcolor{colorCOIGPropertyCounts_Langs}{2} & \cellcolor{colorDialogStudioPropertyCounts_Domains}{3} & \emojiblank\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \NCDataCircle & \greencheck \\
Gretel Text-to-SQL & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorGretelText-to-SQLPropertyCounts_Langs}{3} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
Conifer & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorCidarPropertyCounts_Tasks}{8} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{2} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Cidar & 2024 & \cellcolor{colorCidarPropertyCounts_Datasets}{1} & \cellcolor{colorCidarPropertyCounts_Tasks}{8} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
Aya & 2024 & \cellcolor{colorAyaPropertyCounts_Datasets}{71} & \cellcolor{colorWildChatPropertyCounts_Tasks}{7} & \cellcolor{colorAyaPropertyCounts_Langs}{71} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emoji{globe-with-meridians}\emojiblank & \CommercialDataCircle \TransparentCircle \TransparentCircle & \emojiblank \\
WildChat & 2024 & \cellcolor{colorWildChatPropertyCounts_Datasets}{2} & \cellcolor{colorWildChatPropertyCounts_Tasks}{7} & \cellcolor{colorWildChatPropertyCounts_Langs}{10} & \cellcolor{colorWildChatPropertyCounts_Domains}{1} & \emojiblank\emoji{robot} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Medical Meadow & Mult. & \cellcolor{colorMedicalMeadowPropertyCounts_Datasets}{8} & \cellcolor{colorMedicalMeadowPropertyCounts_Tasks}{2} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorDialogStudioPropertyCounts_Domains}{3} & \emoji{globe-with-meridians}\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \NCDataCircle & \greencheck \\
PMC-LLaMA Instr. & Mult. & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Datasets}{7} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Tasks}{1} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorPMC-LLaMAInstr.PropertyCounts_Domains}{2} & \emoji{globe-with-meridians}\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
DialogStudio & Mult. & \cellcolor{colorDialogStudioPropertyCounts_Datasets}{83} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorDialogStudioPropertyCounts_Langs}{5} & \cellcolor{colorDialogStudioPropertyCounts_Domains}{3} & \emoji{globe-with-meridians}\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \NCDataCircle & \emojiblank \\
COIG & Mult. & \cellcolor{colorCOIGPropertyCounts_Datasets}{18} & \cellcolor{colorCOIGPropertyCounts_Tasks}{13} & \cellcolor{colorCOIGPropertyCounts_Langs}{2} & \cellcolor{colorCOIGPropertyCounts_Domains}{22} & \emoji{globe-with-meridians}\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \NCDataCircle & \emojiblank \\
AgentInstruct & Mult. & \cellcolor{colorAgentInstructPropertyCounts_Datasets}{6} & \cellcolor{colorAgentInstructPropertyCounts_Tasks}{3} & \cellcolor{colorAgentInstructPropertyCounts_Langs}{1} & \cellcolor{colorAgentInstructPropertyCounts_Domains}{7} & \emoji{globe-with-meridians}\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Open-Platypus & Mult. & \cellcolor{colorOpen-PlatypusPropertyCounts_Datasets}{10} & \cellcolor{colorOpen-PlatypusPropertyCounts_Tasks}{10} & \cellcolor{colorOpen-PlatypusPropertyCounts_Langs}{36} & \cellcolor{colorOpen-PlatypusPropertyCounts_Domains}{8} & \emoji{globe-with-meridians}\emoji{robot} & \CommercialDataCircle \UnspecifiedDataCircle \NCDataCircle & \greencheck \\
\end{longtable}

==> tables/collections-video.tex <==
\setlength{\tabcolsep}{1.9pt}
\definecolor{colorHOLLYWOOD2PropertyCounts_Hours}{RGB}{229,241,239}
\definecolor{colorCollectivePropertyCounts_Hours}{RGB}{240,223,178}
\definecolor{colorHMDBPropertyCounts_Hours}{RGB}{204,235,230}
\definecolor{colorUCF101PropertyCounts_Hours}{RGB}{227,240,239}
\definecolor{color50SaladsPropertyCounts_Hours}{RGB}{226,240,238}
\definecolor{colorYouCookPropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorVideoStoryPropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorHollywoodExt.PropertyCounts_Hours}{RGB}{233,242,240}
\definecolor{colorTHUMOSPropertyCounts_Hours}{RGB}{218,238,235}
\definecolor{colorBreakfastPropertyCounts_Hours}{RGB}{224,240,237}
\definecolor{colorSumMePropertyCounts_Hours}{RGB}{242,244,244}
\definecolor{colorSports-1MPropertyCounts_Hours}{RGB}{187,229,223}
\definecolor{colorStoryGraphsPropertyCounts_Hours}{RGB}{235,242,241}
\definecolor{colorTVSumPropertyCounts_Hours}{RGB}{236,243,242}
\definecolor{colorVolleyballPropertyCounts_Hours}{RGB}{240,223,178}
\definecolor{colorActivityNetPropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorMovieQAPropertyCounts_Hours}{RGB}{217,238,235}
\definecolor{colorCharadesPropertyCounts_Hours}{RGB}{224,240,237}
\definecolor{colorMarsPropertyCounts_Hours}{RGB}{240,223,178}
\definecolor{colorMSR-VTTPropertyCounts_Hours}{RGB}{226,240,238}
\definecolor{colorVTWPropertyCounts_Hours}{RGB}{218,238,235}
\definecolor{colorTGIFPropertyCounts_Hours}{RGB}{224,240,237}
\definecolor{colorNTURGB+DPropertyCounts_Hours}{RGB}{224,240,237}
\definecolor{colorNarratedInstr.Vid.PropertyCounts_Hours}{RGB}{235,242,241}
\definecolor{colorYoutube-8MPropertyCounts_Hours}{RGB}{179,226,219}
\definecolor{colorYouCook2PropertyCounts_Hours}{RGB}{220,239,236}
\definecolor{colorMultiTHUMOSPropertyCounts_Hours}{RGB}{227,240,239}
\definecolor{colorImageNet-VidPropertyCounts_Hours}{RGB}{233,242,240}
\definecolor{colorPKU-MMDPropertyCounts_Hours}{RGB}{226,240,238}
\definecolor{color20BN-SOMETHINGPropertyCounts_Hours}{RGB}{222,239,237}
\definecolor{colorVoxCelebPropertyCounts_Hours}{RGB}{209,236,232}
\definecolor{colorQFVSPropertyCounts_Hours}{RGB}{229,241,239}
\definecolor{colorDavisPropertyCounts_Hours}{RGB}{240,223,178}
\definecolor{colorDiDeMoPropertyCounts_Hours}{RGB}{218,238,235}
\definecolor{colorHow2PropertyCounts_Hours}{RGB}{209,236,232}
\definecolor{colorSOAPropertyCounts_Hours}{RGB}{211,237,233}
\definecolor{colorVLOGPropertyCounts_Hours}{RGB}{217,238,235}
\definecolor{colorCharades-EgoPropertyCounts_Hours}{RGB}{224,240,237}
\definecolor{colorEPIC-KITCHENSPropertyCounts_Hours}{RGB}{222,239,237}
\definecolor{colorMovieGraphsPropertyCounts_Hours}{RGB}{222,239,237}
\definecolor{color20BN-jesterPropertyCounts_Hours}{RGB}{231,241,240}
\definecolor{colorCOINPropertyCounts_Hours}{RGB}{215,237,234}
\definecolor{colorCrossTaskPropertyCounts_Hours}{RGB}{217,238,235}
\definecolor{colorToyotaSmarthomePropertyCounts_Hours}{RGB}{218,238,235}
\definecolor{colorVaTeXPropertyCounts_Hours}{RGB}{222,239,237}
\definecolor{colorMSAPropertyCounts_Hours}{RGB}{215,237,234}
\definecolor{colorMMActPropertyCounts_Hours}{RGB}{222,239,237}
\definecolor{colorTRECVidPropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorHACSPropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorHowTo100MPropertyCounts_Hours}{RGB}{187,229,223}
\definecolor{colorMomentsinTimePropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorVIOLINPropertyCounts_Hours}{RGB}{215,237,234}
\definecolor{colorTITANPropertyCounts_Hours}{RGB}{238,243,242}
\definecolor{colorRareActPropertyCounts_Hours}{RGB}{229,241,239}
\definecolor{colorTinyVIRATPropertyCounts_Hours}{RGB}{231,241,240}
\definecolor{color100DOHPropertyCounts_Hours}{RGB}{206,235,231}
\definecolor{colorOops!PropertyCounts_Hours}{RGB}{226,240,238}
\definecolor{colorOmniSource-WebPropertyCounts_Hours}{RGB}{200,234,229}
\definecolor{colorCondensedMoviesPropertyCounts_Hours}{RGB}{211,237,233}
\definecolor{colorMovieScenesPropertyCounts_Hours}{RGB}{218,238,235}
\definecolor{colorMovie-NetPropertyCounts_Hours}{RGB}{208,236,232}
\definecolor{colorEEVPropertyCounts_Hours}{RGB}{217,238,235}
\definecolor{colorFineGymPropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorLEMMAPropertyCounts_Hours}{RGB}{231,241,240}
\definecolor{colorHAA500PropertyCounts_Hours}{RGB}{235,242,241}
\definecolor{colorHVUPropertyCounts_Hours}{RGB}{190,230,224}
\definecolor{colorApesPropertyCounts_Hours}{RGB}{227,240,239}
\definecolor{colorWebVidPropertyCounts_Hours}{RGB}{200,234,229}
\definecolor{colorVideoLTPropertyCounts_Hours}{RGB}{200,234,229}
\definecolor{colorUAV-HumanPropertyCounts_Hours}{RGB}{229,241,239}
\definecolor{colorHD-VILA-100MPropertyCounts_Hours}{RGB}{217,238,235}
\definecolor{colorHOMAGEPropertyCounts_Hours}{RGB}{227,240,239}
\definecolor{colorSpokenMomentsPropertyCounts_Hours}{RGB}{217,238,235}
\definecolor{colorM-MiTPropertyCounts_Hours}{RGB}{213,237,234}
\definecolor{colorQuerYDPropertyCounts_Hours}{RGB}{218,238,235}
\definecolor{colorMimeticsPropertyCounts_Hours}{RGB}{242,244,244}
\definecolor{colorFERV39kPropertyCounts_Hours}{RGB}{231,241,240}
\definecolor{colorMADPropertyCounts_Hours}{RGB}{211,237,233}
\definecolor{colorCDADPropertyCounts_Hours}{RGB}{218,238,235}
\definecolor{colorKineticsPropertyCounts_Hours}{RGB}{206,235,231}
\definecolor{colorLSMDCPropertyCounts_Hours}{RGB}{217,238,235}
\definecolor{colorEgo4DPropertyCounts_Hours}{RGB}{206,235,231}
\definecolor{colorMPIIPropertyCounts_Hours}{RGB}{222,239,237}
\definecolor{colorAvaPropertyCounts_Hours}{RGB}{220,239,236}
\definecolor{colorProject-AriaPropertyCounts_Hours}{RGB}{211,237,233}
\definecolor{colorHOLLYWOOD2PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCollectivePropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHMDBPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorUCF101PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{color50SaladsPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorYouCookPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVideoStoryPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHollywoodExt.PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorTHUMOSPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorBreakfastPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorSumMePropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorSports-1MPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorStoryGraphsPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorTVSumPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVolleyballPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorActivityNetPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMovieQAPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCharadesPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMarsPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMSR-VTTPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVTWPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorTGIFPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorNTURGB+DPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorNarratedInstr.Vid.PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorYoutube-8MPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorYouCook2PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMultiTHUMOSPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorImageNet-VidPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorPKU-MMDPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{color20BN-SOMETHINGPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVoxCelebPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorQFVSPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorDavisPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorDiDeMoPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHow2PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorSOAPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVLOGPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCharades-EgoPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorEPIC-KITCHENSPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMovieGraphsPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{color20BN-jesterPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCOINPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCrossTaskPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorToyotaSmarthomePropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVaTeXPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMSAPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMMActPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorTRECVidPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHACSPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHowTo100MPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMomentsinTimePropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVIOLINPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorTITANPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorRareActPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorTinyVIRATPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{color100DOHPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorOops!PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorOmniSource-WebPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCondensedMoviesPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMovieScenesPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMovie-NetPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorEEVPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorFineGymPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorLEMMAPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHAA500PropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHVUPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorApesPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorWebVidPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorVideoLTPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorUAV-HumanPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHD-VILA-100MPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorHOMAGEPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorSpokenMomentsPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorM-MiTPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorQuerYDPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMimeticsPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorFERV39kPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorMADPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorCDADPropertyCounts_Datasets}{RGB}{240,223,178}
\definecolor{colorKineticsPropertyCounts_Datasets}{RGB}{179,226,219}
\definecolor{colorLSMDCPropertyCounts_Datasets}{RGB}{229,241,239}
\definecolor{colorEgo4DPropertyCounts_Datasets}{RGB}{229,241,239}
\definecolor{colorMPIIPropertyCounts_Datasets}{RGB}{179,226,219}
\definecolor{colorAvaPropertyCounts_Datasets}{RGB}{229,241,239}
\definecolor{colorProject-AriaPropertyCounts_Datasets}{RGB}{229,241,239}
\definecolor{colorHOLLYWOOD2PropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorCollectivePropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHMDBPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorUCF101PropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{color50SaladsPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorYouCookPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorVideoStoryPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHollywoodExt.PropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorTHUMOSPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorBreakfastPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorSumMePropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorSports-1MPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorStoryGraphsPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorTVSumPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorVolleyballPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorActivityNetPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorMovieQAPropertyCounts_Countries}{RGB}{211,237,233}
\definecolor{colorCharadesPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorMarsPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorMSR-VTTPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorVTWPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorTGIFPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorNTURGB+DPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorNarratedInstr.Vid.PropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorYoutube-8MPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorYouCook2PropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorMultiTHUMOSPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorImageNet-VidPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorPKU-MMDPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{color20BN-SOMETHINGPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorVoxCelebPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorQFVSPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorDavisPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorDiDeMoPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHow2PropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorSOAPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorVLOGPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorCharades-EgoPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorEPIC-KITCHENSPropertyCounts_Countries}{RGB}{211,237,233}
\definecolor{colorMovieGraphsPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{color20BN-jesterPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorCOINPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorCrossTaskPropertyCounts_Countries}{RGB}{179,226,219}
\definecolor{colorToyotaSmarthomePropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorVaTeXPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorMSAPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorMMActPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorTRECVidPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHACSPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHowTo100MPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorMomentsinTimePropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorVIOLINPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorTITANPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorRareActPropertyCounts_Countries}{RGB}{211,237,233}
\definecolor{colorTinyVIRATPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{color100DOHPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorOops!PropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorOmniSource-WebPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorCondensedMoviesPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorMovieScenesPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorMovie-NetPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorEEVPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorFineGymPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorLEMMAPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHAA500PropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorHVUPropertyCounts_Countries}{RGB}{211,237,233}
\definecolor{colorApesPropertyCounts_Countries}{RGB}{211,237,233}
\definecolor{colorWebVidPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorVideoLTPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorUAV-HumanPropertyCounts_Countries}{RGB}{245,244,244}
\definecolor{colorHD-VILA-100MPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHOMAGEPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorSpokenMomentsPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorM-MiTPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorQuerYDPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorMimeticsPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorFERV39kPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorMADPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorCDADPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorKineticsPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorLSMDCPropertyCounts_Countries}{RGB}{179,226,219}
\definecolor{colorEgo4DPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorMPIIPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorAvaPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorProject-AriaPropertyCounts_Countries}{RGB}{239,221,175}
\definecolor{colorHOLLYWOOD2PropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorCollectivePropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorHMDBPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorUCF101PropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{color50SaladsPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorYouCookPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorVideoStoryPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorHollywoodExt.PropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorTHUMOSPropertyCounts_Creators}{RGB}{233,242,240}
\definecolor{colorBreakfastPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorSumMePropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorSports-1MPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorStoryGraphsPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorTVSumPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorVolleyballPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorActivityNetPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorMovieQAPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorCharadesPropertyCounts_Creators}{RGB}{233,242,240}
\definecolor{colorMarsPropertyCounts_Creators}{RGB}{233,242,240}
\definecolor{colorMSR-VTTPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorVTWPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorTGIFPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorNTURGB+DPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorNarratedInstr.Vid.PropertyCounts_Creators}{RGB}{233,242,240}
\definecolor{colorYoutube-8MPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorYouCook2PropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorMultiTHUMOSPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorImageNet-VidPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorPKU-MMDPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{color20BN-SOMETHINGPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorVoxCelebPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorQFVSPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorDavisPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorDiDeMoPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorHow2PropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorSOAPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorVLOGPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorCharades-EgoPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorEPIC-KITCHENSPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorMovieGraphsPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{color20BN-jesterPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorCOINPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorCrossTaskPropertyCounts_Creators}{RGB}{222,239,237}
\definecolor{colorToyotaSmarthomePropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorVaTeXPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorMSAPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorMMActPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorTRECVidPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorHACSPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorHowTo100MPropertyCounts_Creators}{RGB}{233,242,240}
\definecolor{colorMomentsinTimePropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorVIOLINPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorTITANPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorRareActPropertyCounts_Creators}{RGB}{222,239,237}
\definecolor{colorTinyVIRATPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{color100DOHPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorOops!PropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorOmniSource-WebPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorCondensedMoviesPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorMovieScenesPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorMovie-NetPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorEEVPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorFineGymPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorLEMMAPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorHAA500PropertyCounts_Creators}{RGB}{233,242,240}
\definecolor{colorHVUPropertyCounts_Creators}{RGB}{222,239,237}
\definecolor{colorApesPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorWebVidPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorVideoLTPropertyCounts_Creators}{RGB}{233,242,240}
\definecolor{colorUAV-HumanPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorHD-VILA-100MPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorHOMAGEPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorSpokenMomentsPropertyCounts_Creators}{RGB}{245,244,242}
\definecolor{colorM-MiTPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorQuerYDPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorMimeticsPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorFERV39kPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorMADPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorCDADPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorKineticsPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorLSMDCPropertyCounts_Creators}{RGB}{179,226,219}
\definecolor{colorEgo4DPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorMPIIPropertyCounts_Creators}{RGB}{245,238,220}
\definecolor{colorAvaPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorProject-AriaPropertyCounts_Creators}{RGB}{240,223,178}
\definecolor{colorHOLLYWOOD2PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorCollectivePropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorHMDBPropertyCounts_Sources}{RGB}{226,240,238}
\definecolor{colorUCF101PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{color50SaladsPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorYouCookPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorVideoStoryPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorHollywoodExt.PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorTHUMOSPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorBreakfastPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorSumMePropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorSports-1MPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorStoryGraphsPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorTVSumPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorVolleyballPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorActivityNetPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMovieQAPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorCharadesPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMarsPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMSR-VTTPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorVTWPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorTGIFPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorNTURGB+DPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorNarratedInstr.Vid.PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorYoutube-8MPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorYouCook2PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMultiTHUMOSPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorImageNet-VidPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorPKU-MMDPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{color20BN-SOMETHINGPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorVoxCelebPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorQFVSPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorDavisPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorDiDeMoPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorHow2PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorSOAPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorVLOGPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorCharades-EgoPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorEPIC-KITCHENSPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMovieGraphsPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{color20BN-jesterPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorCOINPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorCrossTaskPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorToyotaSmarthomePropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorVaTeXPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMSAPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMMActPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorTRECVidPropertyCounts_Sources}{RGB}{245,238,218}
\definecolor{colorHACSPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorHowTo100MPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMomentsinTimePropertyCounts_Sources}{RGB}{179,226,219}
\definecolor{colorVIOLINPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorTITANPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorRareActPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorTinyVIRATPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{color100DOHPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorOops!PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorOmniSource-WebPropertyCounts_Sources}{RGB}{245,243,240}
\definecolor{colorCondensedMoviesPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMovieScenesPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMovie-NetPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorEEVPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorFineGymPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorLEMMAPropertyCounts_Sources}{RGB}{245,238,218}
\definecolor{colorHAA500PropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorHVUPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorApesPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorWebVidPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorVideoLTPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorUAV-HumanPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorHD-VILA-100MPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorHOMAGEPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorSpokenMomentsPropertyCounts_Sources}{RGB}{179,226,219}
\definecolor{colorM-MiTPropertyCounts_Sources}{RGB}{245,238,218}
\definecolor{colorQuerYDPropertyCounts_Sources}{RGB}{245,238,218}
\definecolor{colorMimeticsPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorFERV39kPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMADPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorCDADPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorKineticsPropertyCounts_Sources}{RGB}{245,238,218}
\definecolor{colorLSMDCPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorEgo4DPropertyCounts_Sources}{RGB}{240,223,178}
\definecolor{colorMPIIPropertyCounts_Sources}{RGB}{245,238,218}
\definecolor{colorAvaPropertyCounts_Sources}{RGB}{245,238,218}
\definecolor{colorProject-AriaPropertyCounts_Sources}{RGB}{240,223,178}

\begin{longtable}{lc|ccccc|cc}
\caption[\textbf{Video collections and properties}]{\textbf{Video collections and properties}. Collection properties include numbers of hours of video, datasets, creator institutions, countries of creator institutions, and data sources. The \textsc{Use} column indicates whether a collection includes data freely usable even for commercial purposes (\protect\CommercialDataCircle), data usable only for noncommercial purposes or academic research (\protect\NCDataCircle) and data whose license status is not specified precisely enough to allow us to determine commercial use permissions (\protect\UnspecifiedDataCircle). Note that each collection may have different datasets with one, two, or all three of these statuses. Finally, the \textsc{Avail} column indicates whether a dataset is available online (\greencheck) or has been taken down, usually for legal reasons (\redcross). Datasets are sorted chronologically to highlight trends over time.} \label{tab:collections-video} \\
\toprule
\textsc{Collection} & \textsc{} & \multicolumn{5}{c}{\textsc{Property Counts}} & \multicolumn{2}{c}{\textsc{Permissions}} \\
 & \textsc{\thead{Year}} & \textsc{\thead{Hours}} & \textsc{\thead{Datasets}} & \textsc{\thead{Countries}} & \textsc{\thead{Creators}} & \textsc{\thead{Sources}} & \textsc{\thead{Use}} & \textsc{\thead{Avail}} \\
\midrule
\endfirsthead
\caption[]{\textbf{Video collections and properties}.} \\
\toprule
\textsc{Collection} & \textsc{} & \multicolumn{5}{c}{\textsc{Property Counts}} & \multicolumn{2}{c}{\textsc{Permissions}} \\
 & \textsc{\thead{Year}} & \textsc{\thead{Hours}} & \textsc{\thead{Datasets}} & \textsc{\thead{Countries}} & \textsc{\thead{Creators}} & \textsc{\thead{Sources}} & \textsc{\thead{Use}} & \textsc{\thead{Avail}} \\
\midrule
\endhead
\midrule
\multicolumn{9}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
HOLLYWOOD2 & 2009 & \cellcolor{colorQFVSPropertyCounts_Hours}{20} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Collective & 2009 & - & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
HMDB & 2011 & \cellcolor{colorHMDBPropertyCounts_Hours}{7k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorHMDBPropertyCounts_Sources}{5} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
UCF101 & 2012 & \cellcolor{colorUCF101PropertyCounts_Hours}{26} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
50 Salads & 2013 & \cellcolor{color50SaladsPropertyCounts_Hours}{40} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
YouCook & 2013 & \cellcolor{colorTRECVidPropertyCounts_Hours}{1k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
VideoStory & 2014 & \cellcolor{colorVideoStoryPropertyCounts_Hours}{743} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Hollywood Ext. & 2014 & \cellcolor{colorImageNet-VidPropertyCounts_Hours}{9} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
THUMOS & 2014 & \cellcolor{colorTHUMOSPropertyCounts_Hours}{254} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorVideoLTPropertyCounts_Creators}{4} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Breakfast & 2014 & \cellcolor{colorBreakfastPropertyCounts_Hours}{77} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
SumMe & 2014 & \cellcolor{colorMimeticsPropertyCounts_Hours}{1} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Sports-1M & 2014 & \cellcolor{colorSports-1MPropertyCounts_Hours}{106k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
StoryGraphs & 2014 & \cellcolor{colorNarratedInstr.Vid.PropertyCounts_Hours}{7} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
TVSum & 2015 & \cellcolor{colorTVSumPropertyCounts_Hours}{4} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Volleyball & 2015 & - & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
ActivityNet & 2015 & \cellcolor{colorActivityNetPropertyCounts_Hours}{849} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
MovieQA & 2015 & \cellcolor{colorMovieQAPropertyCounts_Hours}{381} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorApesPropertyCounts_Countries}{3} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \redcross \\
Charades & 2016 & \cellcolor{colorCharadesPropertyCounts_Hours}{82} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorVideoLTPropertyCounts_Creators}{4} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Mars & 2016 & - & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorVideoLTPropertyCounts_Creators}{4} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
MSR-VTT & 2016 & \cellcolor{colorMSR-VTTPropertyCounts_Hours}{41} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
VTW & 2016 & \cellcolor{colorVTWPropertyCounts_Hours}{213} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
TGIF & 2016 & \cellcolor{colorTGIFPropertyCounts_Hours}{86} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
NTU RGB+D & 2016 & \cellcolor{colorNTURGB+DPropertyCounts_Hours}{74} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Narrated Instr. Vid. & 2016 & \cellcolor{colorNarratedInstr.Vid.PropertyCounts_Hours}{7} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorVideoLTPropertyCounts_Creators}{4} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Youtube-8M & 2016 & \cellcolor{colorYoutube-8MPropertyCounts_Hours}{350k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
YouCook2 & 2017 & \cellcolor{colorYouCook2PropertyCounts_Hours}{176} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
MultiTHUMOS & 2017 & \cellcolor{colorHOMAGEPropertyCounts_Hours}{30} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
ImageNet-Vid & 2017 & \cellcolor{colorImageNet-VidPropertyCounts_Hours}{9} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
PKU-MMD & 2017 & \cellcolor{colorOops!PropertyCounts_Hours}{50} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
20BN-SOMETHING & 2017 & \cellcolor{color20BN-SOMETHINGPropertyCounts_Hours}{121} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
VoxCeleb & 2017 & \cellcolor{colorVoxCelebPropertyCounts_Hours}{2k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
QFVS & 2017 & \cellcolor{colorQFVSPropertyCounts_Hours}{20} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Davis & 2017 & - & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
DiDeMo & 2018 & \cellcolor{colorDiDeMoPropertyCounts_Hours}{275} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
How2 & 2018 & \cellcolor{colorHow2PropertyCounts_Hours}{2k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
SOA & 2018 & \cellcolor{colorSOAPropertyCounts_Hours}{2k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
VLOG & 2018 & \cellcolor{colorVLOGPropertyCounts_Hours}{336} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Charades-Ego & 2018 & \cellcolor{colorCharades-EgoPropertyCounts_Hours}{69} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
EPIC-KITCHENS & 2018 & \cellcolor{colorMMActPropertyCounts_Hours}{100} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorApesPropertyCounts_Countries}{3} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
MovieGraphs & 2018 & \cellcolor{colorMovieGraphsPropertyCounts_Hours}{94} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \redcross \\
20BN-jester & 2019 & \cellcolor{color20BN-jesterPropertyCounts_Hours}{13} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
COIN & 2019 & \cellcolor{colorCOINPropertyCounts_Hours}{476} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
CrossTask & 2019 & \cellcolor{colorCrossTaskPropertyCounts_Hours}{376} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorLSMDCPropertyCounts_Countries}{4} & \cellcolor{colorHVUPropertyCounts_Creators}{5} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Toyota Smarthome & 2019 & \cellcolor{colorToyotaSmarthomePropertyCounts_Hours}{269} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
VaTeX & 2019 & \cellcolor{colorVaTeXPropertyCounts_Hours}{115} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
MSA & 2019 & \cellcolor{colorMSAPropertyCounts_Hours}{516} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
MMAct & 2019 & \cellcolor{colorMMActPropertyCounts_Hours}{100} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
TRECVid & 2019 & \cellcolor{colorTRECVidPropertyCounts_Hours}{1k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorAvaPropertyCounts_Sources}{2} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
HACS & 2019 & \cellcolor{colorM-MiTPropertyCounts_Hours}{833} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
HowTo100M & 2019 & \cellcolor{colorHowTo100MPropertyCounts_Hours}{134k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorVideoLTPropertyCounts_Creators}{4} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Moments in Time & 2019 & \cellcolor{colorM-MiTPropertyCounts_Hours}{833} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorSpokenMomentsPropertyCounts_Sources}{11} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
VIOLIN & 2020 & \cellcolor{colorVIOLINPropertyCounts_Hours}{582} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
TITAN & 2020 & \cellcolor{colorTITANPropertyCounts_Hours}{3} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
RareAct & 2020 & \cellcolor{colorRareActPropertyCounts_Hours}{21} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorApesPropertyCounts_Countries}{3} & \cellcolor{colorHVUPropertyCounts_Creators}{5} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
TinyVIRAT & 2020 & \cellcolor{colorLEMMAPropertyCounts_Hours}{11} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
100DOH & 2020 & \cellcolor{color100DOHPropertyCounts_Hours}{5k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Oops! & 2020 & \cellcolor{colorOops!PropertyCounts_Hours}{50} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
OmniSource-Web & 2020 & \cellcolor{colorOmniSource-WebPropertyCounts_Hours}{13k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorOmniSource-WebPropertyCounts_Sources}{3} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Condensed Movies & 2020 & \cellcolor{colorCondensedMoviesPropertyCounts_Hours}{1k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
MovieScenes & 2020 & \cellcolor{colorMovieScenesPropertyCounts_Hours}{250} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Movie-Net & 2020 & \cellcolor{colorMovie-NetPropertyCounts_Hours}{3k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
EEV & 2020 & \cellcolor{colorEEVPropertyCounts_Hours}{370} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
FineGym & 2020 & \cellcolor{colorFineGymPropertyCounts_Hours}{708} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
LEMMA & 2020 & \cellcolor{colorLEMMAPropertyCounts_Hours}{11} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorAvaPropertyCounts_Sources}{2} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
HAA500 & 2020 & \cellcolor{colorHAA500PropertyCounts_Hours}{5} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorVideoLTPropertyCounts_Creators}{4} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
HVU & 2020 & \cellcolor{colorHVUPropertyCounts_Hours}{96k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorApesPropertyCounts_Countries}{3} & \cellcolor{colorHVUPropertyCounts_Creators}{5} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Apes & 2021 & \cellcolor{colorApesPropertyCounts_Hours}{36} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorApesPropertyCounts_Countries}{3} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
WebVid & 2021 & \cellcolor{colorWebVidPropertyCounts_Hours}{13k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \redcross \\
VideoLT & 2021 & \cellcolor{colorVideoLTPropertyCounts_Hours}{14k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorVideoLTPropertyCounts_Creators}{4} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
UAV-Human & 2021 & \cellcolor{colorUAV-HumanPropertyCounts_Hours}{18} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorUAV-HumanPropertyCounts_Countries}{2} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
HD-VILA-100M & 2021 & \cellcolor{colorHD-VILA-100MPropertyCounts_Hours}{372} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
HOMAGE & 2021 & \cellcolor{colorHOMAGEPropertyCounts_Hours}{30} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Spoken Moments & 2021 & \cellcolor{colorSpokenMomentsPropertyCounts_Hours}{417} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorSpokenMomentsPropertyCounts_Creators}{3} & \cellcolor{colorSpokenMomentsPropertyCounts_Sources}{11} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
M-MiT & 2021 & \cellcolor{colorM-MiTPropertyCounts_Hours}{833} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorAvaPropertyCounts_Sources}{2} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
QuerYD & 2021 & \cellcolor{colorQuerYDPropertyCounts_Hours}{207} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorAvaPropertyCounts_Sources}{2} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Mimetics & 2021 & \cellcolor{colorMimeticsPropertyCounts_Hours}{1} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
FERV39k & 2022 & \cellcolor{colorFERV39kPropertyCounts_Hours}{16} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \TransparentCircle \NCDataCircle & \greencheck \\
MAD & 2022 & \cellcolor{colorMADPropertyCounts_Hours}{1k} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
CDAD & 2022 & \cellcolor{colorCDADPropertyCounts_Hours}{215} & \cellcolor{colorCDADPropertyCounts_Datasets}{1} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Kinetics & Mult. & \cellcolor{colorKineticsPropertyCounts_Hours}{4k} & \cellcolor{colorMPIIPropertyCounts_Datasets}{3} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorAvaPropertyCounts_Sources}{2} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
LSMDC & Mult. & \cellcolor{colorLSMDCPropertyCounts_Hours}{316} & \cellcolor{colorProject-AriaPropertyCounts_Datasets}{2} & \cellcolor{colorLSMDCPropertyCounts_Countries}{4} & \cellcolor{colorLSMDCPropertyCounts_Creators}{10} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Ego4D & Mult. & \cellcolor{colorEgo4DPropertyCounts_Hours}{5k} & \cellcolor{colorProject-AriaPropertyCounts_Datasets}{2} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
MPII & Mult. & \cellcolor{colorMPIIPropertyCounts_Hours}{110} & \cellcolor{colorMPIIPropertyCounts_Datasets}{3} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorMPIIPropertyCounts_Creators}{2} & \cellcolor{colorAvaPropertyCounts_Sources}{2} & \TransparentCircle \UnspecifiedDataCircle \TransparentCircle & \greencheck \\
Ava & Mult. & \cellcolor{colorAvaPropertyCounts_Hours}{146} & \cellcolor{colorProject-AriaPropertyCounts_Datasets}{2} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorAvaPropertyCounts_Sources}{2} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
Project-Aria & Mult. & \cellcolor{colorProject-AriaPropertyCounts_Hours}{1k} & \cellcolor{colorProject-AriaPropertyCounts_Datasets}{2} & \cellcolor{colorProject-AriaPropertyCounts_Countries}{1} & \cellcolor{colorProject-AriaPropertyCounts_Creators}{1} & \cellcolor{colorProject-AriaPropertyCounts_Sources}{1} & \CommercialDataCircle \TransparentCircle \TransparentCircle & \greencheck \\
\end{longtable}

==> tables/refs-licenses-audio.tex <==
\begin{longtable}{p{5cm}|p{5cm}|p{5cm}}
\caption[\textbf{References and licenses: audio}]{\textbf{References and licenses for audio} dataset collections presented in this paper. Collections containing material under more than three distinct licenses are marked as having ``Various'' licenses, and we refer readers to our raw data for the full details. Datasets are sorted alphabetically for ease of dataset lookup.} \label{tab:refs-licenses-audio} \\
\toprule
Collection & Licenses & Cite \\
\midrule
\endfirsthead
\caption[]{\textbf{References and licenses for audio}.} \\
\toprule
Collection & Licenses & Cite \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
1111 Hours Hindi & Custom & \cite{bhanushaliGramVaaniASR2022} \\
120h Spanish Speech & CC0 1.0 & -- \\
AFRISPEECH-200 & CC BY-NC-SA 4.0 & \cite{olatunjiAfriSpeech200PanAfricanAccented2023} \\
AISHELL-1 & Apache 2.0 & \cite{buAISHELL1OpenSourceMandarin2017} \\
AISHELL-2 & Unspecified & \cite{duAISHELL2TransformingMandarin2018} \\
AISHELL-4 & CC BY-SA 4.0 & \cite{fuAISHELL4OpenSource2021} \\
ALLSSTAR & CC BY 4.0 & \cite{bradlowALLSSTARArchiveL12010} \\
AMI & CC BY 4.0 & \cite{carlettaAMIMeetingCorpus2006} \\
Aalto Finnish Parl. & Custom & \cite{virkkunenFinnishParliamentASR2022} \\
African Acc. French & Apache 2.0 & -- \\
Basq., Cat. and Gal. & CC BY-SA 4.0 & \cite{kjartanssonOpenSourceHighQuality2020} \\
Bloom Speech & Various & \cite{leongBloomLibraryMultimodal2022} \\
Bud500 & Apache 2.0, CC BY-NC-SA 4.0 & -- \\
CSJ & Custom & \cite{maekawaCorpusSpontaneousJapanese2003} \\
CSLU 1.2 & CSLU Agreement & \cite{landertCSLUForeignAccented2007} \\
CSLU 22 Langs. & CSLU Agreement & \cite{landertCSLU22Languages2005} \\
ClarinPL & CC BY 4.0 & \cite{korzinekPolishReadSpeech2017} \\
CoNASE & Custom & \cite{coatsCorpusRegionalAmerican2019} \\
CoVoST-2 & CC0 1.0 & \cite{wangCoVoSTMassivelyMultilingual2020} \\
Common Voice 17 & CC0 1.0 & \cite{ardilaCommonVoiceMassivelyMultilingual2020} \\
Crowd Sourced Speech & CC BY-SA 4.0 & \cite{kjartanssonCrowdSourcedSpeechCorpora2018} \\
Czech Parliament & CC BY 4.0 & \cite{kratochvilLargeCorpusCzech2020} \\
DiDiSpeech & Unspecified & \cite{guoDiDiSpeechLargeScale2021} \\
Earnings-22 & Unspecified & \cite{delrioEarnings22PracticalBenchmark2022} \\
EdAcc & CC BY-SA 4.0 & \cite{sanabriaEdinburghInternationalAccents2023} \\
Eng. Acc. in Brit. Isles & CC BY-SA 4.0 & \cite{demirsahinOpensourceMultispeakerCorpora2020} \\
English-Vietnamese & CC BY-NC-ND 4.0 & \cite{nguyenHighQualityLargeScaleDataset2022} \\
FT SPEECH & Custom & \cite{kirkedalFTSpeechDanish2020} \\
Fisher & LDC User Agreement & \cite{cieriFisherCorpusResource2004} \\
Fleurs & CC BY 4.0 & \cite{conneauFLEURSFewshotLearning2022} \\
GigaSpeech & Apache 2.0 & \cite{chenGigaSpeechEvolvingMultidomain2021} \\
Golos & Custom & \cite{karpovGolosRussianDataset2021} \\
Hebrew Coursera & Unspecified & -- \\
Hebrew Kan & Unspecified & -- \\
Highland Puebla Nahuatl & CC BY-NC-SA 3.0 & \cite{shiHighlandPueblaNahuatl2021} \\
JTUBESPEECH & Unspecified & \cite{takamichiJTubeSpeechCorpusJapanese2021} \\
Japanese Anime Speech & CC0 1.0 & -- \\
KSC & CC BY 4.0 & \cite{khassanovCrowdsourcedOpenSourceKazakh2021} \\
Kathbath & CC0 1.0 & \cite{javedIndicSUPERBSpeechProcessing2022} \\
KeSpeech & Custom & \cite{tangKeSpeechOpenSource2021} \\
KsponSpeech & Unspecified & \cite{bangKsponSpeechKoreanSpontaneous2020} \\
LJSpeech & Public Domain & \cite{itoLJSpeechDataset2017} \\
LaboroTVSpeech & Custom & \cite{andoConstructionLargescaleJapanese2021} \\
LibriSpeech & CC BY 4.0 & \cite{panayotovLibrispeechASRCorpus2015} \\
M-AILABS & Custom & \cite{solakMAILABSSpeechDataset2024} \\
M2ASR & Unspecified & \cite{shiFreeKazakhSpeech2017,mamtiminM2ASRKIRGHIZFreeKirghiz2023,zhiM2ASRMONGOFreeMongolian2021,liFreeLinguisticSpeech2017} \\
MAGICDATA & CC BY-NC-ND 4.0 & -- \\
MASC & CC BY 4.0 & \cite{al-fetyaniMASCMassiveArabic2023} \\
MaSS & Unspecified & \cite{boitoMaSSLargeClean2020} \\
MagicData-RAMC & CC BY-NC-ND 4.0 & \cite{yangOpenSourceMagicDataRAMC2022} \\
MediaSpeech & CC BY 4.0 & \cite{kolobovMediaSpeechMultilanguageASR2021} \\
Minds14 & CC BY 4.0 & \cite{gerzMultilingualCrossLingualIntent2021} \\
MuST-C & CC BY-NC-ND 4.0 & \cite{digangiMuSTCMultilingualSpeech2019} \\
Multiling. LibriSpeech & CC BY 4.0 & \cite{pratapMLSLargeScaleMultilingual2020} \\
Multiling. TEDx & CC BY-NC-ND 4.0 & \cite{saleskyMultilingualTEDxCorpus2021} \\
NST Danish & CC0 1.0 & -- \\
NST Norwegian & CC0 1.0 & -- \\
NST Swedish & CC0 1.0 & -- \\
Nigerian English & CC BY-SA 4.0 & -- \\
Norwegian Parl. & CC0 1.0 & \cite{solbergNorwegianParliamentarySpeech2022} \\
Norwegian Parl. Speech & CC0 1.0 & \cite{solbergNorwegianParliamentarySpeech2022} \\
OLKAVS & Custom & \cite{parkOLKAVSOpenLargeScale2023} \\
OpenSTT & CC BY-NC 4.0 & \cite{andrusenkoExplorationEndtoEndASR2020} \\
People's Speech & Various & \cite{galvezPeopleSpeechLargeScale2021} \\
QASR & Unspecified & \cite{mubarakQASRQCRIAljazeera2021} \\
RTVE & Custom & -- \\
ReazonSpeech & CDLA-Sharing-1.0 & \cite{yinReazonSpeechFreeMassive2023} \\
Regional Af. Am. Lang. & CC BY-NC-SA 4.0 & -- \\
RixVox & CC BY 4.0 & -- \\
SDS-200 & Custom & \cite{plussSDS200SwissGerman2022} \\
SPGISpeech & Custom & \cite{oneillSPGISpeech000Hours2021} \\
Samromur & CC BY 4.0 & \cite{mollbergSamromurCrowdsourcingData2020} \\
Samromur Children & CC BY 4.0 & \cite{hernandezmenaSamromurChildrenIcelandic2022} \\
Samromur Milljon & CC BY 4.0 & -- \\
Shrutilipi & CC0 1.0 & \cite{bhogaleEffectivenessMiningAudio2022} \\
Snow Mountain & CC BY-SA 4.0 & \cite{rajuSnowMountainDataset2023} \\
Spoken Wikipedia & CC BY-SA 4.0 & \cite{baumannSpokenWikipediaCorpus2019} \\
Switchboard & LDC User Agreement & \cite{godfreySWITCHBOARDTelephoneSpeech1992} \\
TED-LIUM3 & CC BY-NC-ND 3.0 & \cite{hernandezTEDLIUMTwiceMuch2018} \\
THCHS-30 & Apache 2.0 & \cite{wangTHCHS30FreeChinese2015} \\
THUYG-20 & Apache 2.0 & \cite{roziOpenFreeDatabase2015} \\
TIMIT & LDC User Agreement & \cite{garofolojohns.TIMITAcousticPhoneticContinuous1993} \\
VCTK & CC BY 4.0 & -- \\
VibraVox & CC BY 4.0 & -- \\
VoxPopuli & CC0 1.0 & \cite{wangVoxPopuliLargeScaleMultilingual2021} \\
Vystadial & CC BY-SA 3.0 & \cite{korvasFreeEnglishCzech2014} \\
WenetSpeech & CC BY 4.0 & \cite{zhangWenetSpeech10000Hours2022} \\
West Afr. Radio & CC BY-SA 4.0 & \cite{doumbouyaUsingRadioArchives2021} \\
West Afr. Virt. Asst. & CC BY-SA 4.0 & \cite{doumbouyaUsingRadioArchives2021} \\
YODAS & CC BY 3.0 & \cite{liYodasYoutubeOrientedDataset2023} \\
Zeroth-Korean & CC BY 4.0 & -- \\
aidatatang & CC BY-NC-ND 4.0 & -- \\
\end{longtable}

==> tables/refs-licenses-text.tex <==
\begin{longtable}{p{5cm}|p{5cm}|p{5cm}}
\caption[\textbf{References and licenses: alignment tuning (text}]{\textbf{References and licenses for alignment-tuning (text)} dataset collections presented in this paper. Collections containing material under more than three distinct licenses are marked as having ``Various'' licenses, and we refer readers to our raw data for the full details. Datasets are sorted alphabetically for ease of dataset lookup.} \label{tab:refs-licenses-text} \\
\toprule
Collection & Licenses & Cite \\
\midrule
\endfirsthead
\caption[]{\textbf{References and licenses for alignment-tuning (text)}.} \\
\toprule
Collection & Licenses & Cite \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
10k Prompt Ranked & Unspecified & -- \\
AgentInstruct & CC BY 4.0, Unspecified, MIT License & \cite{shridharALFWorldAligningText2021,yaoWebShopScalableRealWorld2023,liuAgentBenchEvaluatingLLMs2023,zengAgentTuningEnablingGeneralized2023,dengMind2WebGeneralistAgent2023} \\
Aya & Apache License 2.0 & \cite{singhAyaDatasetOpenAccess2024} \\
Bactrian-X & CC BY-SA 3.0, CC BY-NC 4.0 & \cite{liBactrianXMultilingualReplicable2023} \\
COBRA Frames & BigScience OpenRAIL-M & \cite{zhouCOBRAFramesContextual2023} \\
COIG & Various & \cite{zhangChineseOpenInstruction2023,baiCOIGCQIAQualityAll2024} \\
Capybara & Various & -- \\
ChatDoctor & Unspecified & \cite{liChatDoctorMedicalChat2023} \\
ChatbotArena & CC BY 4.0, CC BY-NC 4.0 & \cite{zhengJudgingLLMasaJudgeMTBench2023} \\
Cidar & CC BY-NC 4.0 & \cite{alyafeaiCIDARCulturallyRelevant2024} \\
CollectiveCognition & MIT License & -- \\
Conifer & Apache License 2.0 & \cite{sunConiferImprovingComplex2024} \\
Deita 10K & CC BY-NC 4.0, Apache License 2.0 & \cite{liuWhatMakesGood2024} \\
DialogStudio & Various & \cite{chenActionBasedConversationsDataset2021,weiAirDialogueEnvironmentGoalOriented2018,linBiToDBilingualMultiDomain2021,chawlaCaSiNoCorpusCampsite2021,heDecouplingStrategyGeneration2018,mrksicNeuralBeliefTracker2017,qianDatabaseSearchResults2022,liuDuRecDialBilingualParallel2021,elasriFramesCorpusAdding2017,quanGECOREndtoEndGenerative2019,chenSemanticallyConditionedDialog2019a,chenKETODKnowledgeEnrichedTaskOriented2022,ericKeyValueRetrievalNetworks2017,zangMultiWOZDialogueDataset2020,shalyminovFewShotDialogueGeneration2019,martinMuDoCoCorpusMultidomain2020,peskovMultiDomainGoalOrientedDialogues2019,ericMultiWOZConsolidatedMultiDomain2019,moonOpenDialKGExplainableConversational2019,rastogiScalableMultidomainConversational2020,mosigSTARSchemaGuidedDialog2020,chiuSalesBotTransitioningChitChat2022,shahBuildingConversationalAgent2018,byrneTaskmaster1RealisticDiverse2019,mrksicFullyStatisticalNeural2018,shangUnsupervisedAbstractiveMeeting2018,rameshkumarStorytellingDialogueCritical2020,fabbriConvoSummConversationSummarization2021,chenDialogSumRealLifeScenario2021,mukherjeeECTSumNewBenchmark2022,shangUnsupervisedAbstractiveMeeting2018,zhuMediaSumLargescaleMedia2021,zhongQMSumNewBenchmark2021,gliwaSAMSumCorpusHumanannotated2019,chenSummScreenDatasetAbstractive2022,feigenblatTWEETSUMMDialogSummarization2021,liEndtoEndTrainableNonCollaborative2019,dinanSecondConversationalIntelligence2019,rashkinEmpatheticOpendomainConversation2019,baiTrainingHelpfulHarmless2022,chenPLACESPromptingLanguage2023,kimProsocialDialogProsocialBackbone2022,myersConversationalScaffoldingAnalogybased2020,reddyCoQAConversationalQuestion2019,yuCoSQLConversationalTexttoSQL2019,talmorWebKnowledgeBaseAnswering2018,nanDARTOpenDomainStructured2021,nanFeTaQAFreeformTable2022,guThreeLevelsGeneralization2021,chenHybridQADatasetMultiHop2020,guptaMMQAMultidomainMultilingual2018,liMTOPComprehensiveMultilingual2021,talmorMultiModalQAComplexQuestion2021,yuSParCCrossDomainSemantic2019,iyyerSearchbasedNeuralStructured2017,yuSpiderLargeScaleHumanLabeled2019,parikhToTToControlledTableToText2020,yihValueSemanticParse2016,zhongSeq2SQLGeneratingStructured2017,pasupatCompositionalSemanticParsing2015,komeiliInternetAugmentedDialogueGeneration2022,dinanWizardWikipediaKnowledgePowered2019,hemphillATISSpokenLanguage1990,casanuevaEfficientIntentDetection2020,zhangArePretrainedTransformers2022,larsonEvaluationDatasetIntent2019,rastogiScalableMultidomainConversational2020,liuBenchmarkingNaturalLanguage2019,liuAsgardPortableArchitecture2013,coopeSpanConveRTFewshotSpan2020,couckeSnipsVoicePlatform2018,guptaSemanticParsingTask2018} \\
EverythingLM & MIT License & -- \\
ExpertQA & MIT License & \cite{malaviyaExpertQAExpertCuratedQuestions2024} \\
Feedback Coll. & MIT License & \cite{kimPrometheusInducingFinegrained2024} \\
Glaive Code Asst. & Apache License 2.0 & -- \\
Gretel Text-to-SQL & Apache License 2.0 & -- \\
HelpSteer & CC BY 4.0 & \cite{wangHelpSteerMultiattributeHelpfulness2023} \\
Indic-Instr. & Various & \cite{galaAiravataIntroducingHindi2024} \\
KIWI & CC BY-SA 4.0 & \cite{xuKIWIDatasetKnowledgeIntensive2024} \\
LMSYS-Chat-1M & Anthropic, LMSYS-Chat-1M Dataset License, Llama 2 & \cite{zhengLMSYSChat1MLargeScaleRealWorld2024} \\
Llama2-MedTuned-Instr. & CC BY-NC 4.0 & \cite{rohanianExploringEffectivenessInstruction2023} \\
LongAlign-10k & Anthropic, Apache License 2.0 & \cite{baiLongAlignRecipeLong2024} \\
MathDial & MIT License, CC BY-SA 4.0 & \cite{macinaMathDialDialogueTutoring2023} \\
MathInstr. & MIT License & \cite{yueMAmmoTHBuildingMath2023} \\
MedInstr. & Unspecified & \cite{zhangAlpaCareInstructiontunedLarge2024} \\
Medical Meadow & Various & \cite{hanMedAlpacaOpenSourceCollection2023,wangCORD19COVID19Open2020,jinWhatDiseaseDoes2020,saveryQuestionDrivenSummarizationAnswers2020} \\
MegaWika & CC BY-SA 4.0 & \cite{barhamMegaWikaMillionsReports2023} \\
MetaMathQA & MIT License & \cite{yuMetaMathBootstrapYour2023} \\
Nectar & Various & -- \\
No Robots & CC BY-NC 4.0 & -- \\
Open Asst. v2 & Apache License 2.0 & \cite{kopfOpenAssistantConversationsDemocratizing2023} \\
Open-Platypus & Various & \cite{sawadaARBAdvancedReasoning2023,dettmersQLoRAEfficientFinetuning2023,lightmanLetVerifyStep2023a,yuReClorReadingComprehension2020,wangSciBenchEvaluatingCollegeLevel2024,luLearnExplainMultimodal2022,chenTheoremQATheoremdrivenQuestion2023} \\
OpenGPT Healthcare & Unspecified, OGL 3.0 & -- \\
OpenMathInstr.-1 & Custom, Apache License 2.0, MIT License & \cite{toshniwalOpenMathInstruct1MillionMath2024} \\
Orca-Math & Various & \cite{mitraOrcaMathUnlockingPotential2024} \\
PII-Masking-200k & Non Commercial & -- \\
PMC-LLaMA Instr. & Unspecified, Apache License 2.0 & \cite{wuPMCLLaMABuildingOpensource2023,jinPubMedQADatasetBiomedical2019} \\
Pure-Dove & Apache License 2.0 & -- \\
PygmalionAI-PIPPA & Apache License 2.0 & \cite{goslingPIPPAPartiallySynthetic2023} \\
RiddleSense & MIT License & \cite{linRiddleSenseReasoningRiddle2021} \\
SeaBench & Apache License 2.0 & \cite{nguyenSeaLLMsLargeLanguage2023} \\
SelFee & MIT License & \cite{yeSelFeeIterativeSelfRevising2023} \\
Thai Gen AI & Various & -- \\
UltraChat-200k & CC BY-NC 4.0 & \cite{dingEnhancingChatLanguage2023} \\
UltraFeedback Argilla & Various & -- \\
WildChat & AI2 ImpACT License - Low Risk & \cite{zhaoWildChat1MChatGPT2023} \\
\end{longtable}


==> tables/refs-licenses-video.tex <==
\begin{longtable}{p{5cm}|p{5cm}|p{5cm}}
\caption[\textbf{References and licenses: video}]{\textbf{References and licenses for video} dataset collections presented in this paper. Collections containing material under more than three distinct licenses are marked as having ``Various'' licenses, and we refer readers to our raw data for the full details. Datasets are sorted alphabetically for ease of dataset lookup.} \label{tab:refs-licenses-video} \\
\toprule
Collection & Licenses & Cite \\
\midrule
\endfirsthead
\caption[]{\textbf{References and licenses for video}.} \\
\toprule
Collection & Licenses & Cite \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
100DOH & Custom & \cite{shanUnderstandingHumanHands2020} \\
20BN-SOMETHING & Custom & \cite{goyalSomethingSomethingVideo2017} \\
20BN-jester & Custom & \cite{materzynskaJesterDatasetLargeScale2019} \\
50 Salads & CC BY-NC-SA 4.0 & \cite{steinCombiningEmbeddedAccelerometers2013} \\
ActivityNet & MIT License & \cite{heilbronActivityNetLargescaleVideo2015} \\
Apes & Unspecified & \cite{alcazarAPESAudiovisualPerson2021} \\
Ava & CC BY 4.0 & \cite{rothAVAActiveSpeakerAudioVisualDataset2019,guAVAVideoDataset2018} \\
Breakfast & CC BY 4.0 & \cite{kuehneLanguageActionsRecovering2014} \\
CDAD & Unspecified & \cite{xiangCDADCommonDaily2022} \\
COIN & Custom & \cite{tangCOINLargescaleDataset2019} \\
Charades & Custom & \cite{sigurdssonHollywoodHomesCrowdsourcing2016} \\
Charades-Ego & Custom & \cite{sigurdssonActorObserverJoint2018} \\
Collective & Unspecified & \cite{wongunchoiWhatAreThey2009} \\
Condensed Movies & CC BY 4.0 & \cite{bainCondensedMoviesStory2020} \\
CrossTask & Unspecified & \cite{zhukovCrosstaskWeaklySupervised2019} \\
Davis & Custom & \cite{perazziBenchmarkDatasetEvaluation2016} \\
DiDeMo & BSD 2-Clause License & \cite{hendricksLocalizingMomentsVideo2018} \\
EEV & CC BY 4.0 & \cite{sunEEVLargeScaleDataset2021} \\
EPIC-KITCHENS & CC BY-NC 4.0 & \cite{damenScalingEgocentricVision2018} \\
Ego4D & Custom, MIT License & \cite{graumanEgo4DWorld0002022} \\
FERV39k & CC BY-NC 4.0 & \cite{wangFERV39kLargeScaleMultiScene2022} \\
FineGym & CC BY-NC 4.0 & \cite{shaoFineGymHierarchicalVideo2020} \\
HAA500 & Unspecified & \cite{chungHAA500HumanCentricAtomic2021} \\
HACS & Custom & \cite{zhaoHACSHumanAction2019} \\
HD-VILA-100M & Custom & \cite{xueAdvancingHighResolutionVideoLanguage2022} \\
HMDB & CC BY 4.0 & \cite{kuehneHMDBLargeVideo2011} \\
HOLLYWOOD2 & Unspecified & \cite{marszalekActionsContext2009} \\
HOMAGE & Unspecified & \cite{raiHomeActionGenome2021} \\
HVU & Custom & \cite{dibaLargeScaleHolistic2020} \\
Hollywood Ext. & MIT License & \cite{bojanowskiWeaklySupervisedAction2014} \\
How2 & Various & \cite{sanabriaHow2LargescaleDataset2018} \\
HowTo100M & Unspecified & \cite{miechHowTo100MLearningTextVideo2019} \\
ImageNet-Vid & CC BY-NC 4.0 & \cite{russakovskyImageNetLargeScale2015} \\
Kinetics & Unspecified & \cite{kayKineticsHumanAction2017,carreiraShortNoteKinetics6002018,smairaShortNoteKinetics70020202020} \\
LEMMA & Unspecified & \cite{jiaLEMMAMultiviewDataset2020} \\
LSMDC & Custom, MIT License & \cite{rohrbachMovieDescription2016,sharmaDeepMultimodalFeature2020} \\
M-MiT & Unspecified & \cite{monfortMultiMomentsTimeLearning2021} \\
MAD & Custom & \cite{soldanMADScalableDataset2022} \\
MMAct & Custom & \cite{kongMMActLargeScaleDataset2019} \\
MPII & Custom, Unspecified & \cite{rohrbachRecognizingFineGrainedComposite2016,rohrbachDatasetMovieDescription2015} \\
MSA & Unspecified & \cite{xiongGraphBasedFrameworkBridge2019} \\
MSR-VTT & Unspecified & \cite{xuMSRVTTLargeVideo2016} \\
Mars & Unspecified & \cite{zhengMARSVideoBenchmark2016} \\
Mimetics & Unspecified & \cite{weinzaepfelMimeticsUnderstandingHuman2021} \\
Moments in Time & Custom & \cite{monfortMomentsTimeDataset2019} \\
Movie-Net & Unspecified & \cite{huangMovieNetHolisticDataset2020} \\
MovieGraphs & Custom & \cite{vicolMovieGraphsUnderstandingHumanCentric2018} \\
MovieQA & Unspecified & \cite{tapaswiMovieQAUnderstandingStories2016} \\
MovieScenes & Unspecified & \cite{raoLocaltoGlobalApproachMultimodal2020} \\
MultiTHUMOS & CC BY 4.0 & \cite{yeungEveryMomentCounts2017} \\
NTU RGB+D & Custom & \cite{shahroudyNTURGBLarge2016} \\
Narrated Instr. Vid. & MIT License & \cite{alayracUnsupervisedLearningNarrated2016} \\
OmniSource-Web & Apache License 2.0 & \cite{duanOmnisourcedWeblysupervisedLearning2020} \\
Oops! & CC BY-NC-SA 4.0 & \cite{epsteinOopsPredictingUnintentional2020} \\
PKU-MMD & Unspecified & \cite{liuPKUMMDLargeScale2017} \\
Project-Aria & Apache License 2.0 & \cite{panAriaDigitalTwin2023,lvAriaEverydayActivities2024} \\
QFVS & Unspecified & \cite{sharghiQueryFocusedVideoSummarization2017} \\
QuerYD & Unspecified & \cite{oncescuQuerYDVideoDataset2021} \\
RareAct & Unspecified & \cite{miechRareActVideoDataset2020} \\
SOA & Unspecified & \cite{dibaLargeScaleHolistic2020} \\
Spoken Moments & Custom & \cite{monfortSpokenMomentsLearning2021} \\
Sports-1M & CC BY 3.0 & \cite{karpathyLargeScaleVideoClassification2014} \\
StoryGraphs & Unspecified & \cite{tapaswiStoryGraphsVisualizingCharacter2014} \\
SumMe & Unspecified & \cite{gygliCreatingSummariesUser2014} \\
TGIF & Custom & \cite{liTGIFNewDataset2016} \\
THUMOS & Custom & \cite{idreesTHUMOSChallengeAction2017} \\
TITAN & Non Commercial & \cite{mallaTITANFutureForecast2020} \\
TRECVid & CC BY-NC-SA 4.0 & \cite{awadTRECVID2019Evaluation2020} \\
TVSum & CC BY 3.0 & \cite{yalesongTVSumSummarizingWeb2015} \\
TinyVIRAT & Unspecified & \cite{demirTinyVIRATLowresolutionVideo2020} \\
Toyota Smarthome & Custom & \cite{dasToyotaSmarthomeRealWorld2019} \\
UAV-Human & Custom & \cite{liUAVHumanLargeBenchmark2021} \\
UCF101 & Unspecified & \cite{soomroUCF101Dataset1012012} \\
VIOLIN & Unspecified & \cite{liuVIOLINLargeScaleDataset2020} \\
VLOG & Custom & \cite{fouheyLifestyleVlogsEveryday2017} \\
VTW & Unspecified & \cite{zengTitleGenerationUser2016} \\
VaTeX & CC BY 4.0 & \cite{wangVATEXLargeScaleHighQuality2020} \\
VideoLT & Non Commercial & \cite{zhangVideoLTLargescaleLongtailed2021} \\
VideoStory & Unspecified & \cite{habibianVideoStoryNewMultimedia2014} \\
Volleyball & Unspecified & \cite{ibrahimHierarchicalDeepTemporal2016} \\
VoxCeleb & Custom & \cite{nagraniVoxCelebLargescaleSpeaker2018} \\
WebVid & Custom & \cite{bainFrozenTimeJoint2022} \\
YouCook & Unspecified & \cite{dasThousandFramesJust2013} \\
YouCook2 & MIT License & \cite{zhouAutomaticLearningProcedures2017} \\
Youtube-8M & Unspecified & \cite{abu-el-haijaYouTube8MLargeScaleVideo2016} \\
\end{longtable}
